Rethinking Vision Transformers for MobileNet Size and Speed

With the success of Vision Transformers (ViTs) in computer vision tasks, recent arts try to optimize the performance and complexity of ViTs to enable efficient deployment on mobile devices. Multiple approaches are proposed to accelerate attention mechanism, improve inefficient designs, or incorporate mobile-friendly lightweight convolutions to form hybrid architectures. However, ViT and its variants still have higher latency or considerably more parameters than lightweight CNNs, even true for the years-old MobileNet. In practice, latency and size are both crucial for efficient deployment on resource-constraint hardware. In this work, we investigate a central question, can transformer models run as fast as MobileNet and maintain a similar size? We revisit the design choices of ViTs and propose a novel supernet with low latency and high parameter efficiency. We further introduce a novel fine-grained joint search strategy for transformer models that can find efficient architectures by optimizing latency and number of parameters simultaneously. The proposed models, EfficientFormerV2, achieve 3.5% higher top-1 accuracy than MobileNetV2 on ImageNet-1K with similar latency and parameters. This work demonstrate that properly designed and optimized vision transformers can achieve high performance even with MobileNet-level size and speed.

==> backup/supp_2_downstream.tex <==
\begin{table*}[]
\centering
% \small
\caption{
\textbf{Object detection \&
instance segmentation} on MS COCO 2017. We benchmark on Mask RCNN pipeline. \dagger~refers to the results obtained from the enhanced training recipe. }
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{c|c|cccccc}
% \toprule
% \multirow{2}{*}{Backbone} & \multirow{2}{*}{Params (M)} & \multicolumn{6}{c}{Detection \& Instance Segmentation}  \\ \cline{3-8}
%                           &                         & AP$^{box}$    & AP$^{box}_{50}$   & AP$^{box}_{75}$   & AP$^{mask}$    & AP$^{mask}_{50}$   & AP$^{mask}_{75}$      \\
%                           \hline
%                           \hline
% ResNet18                  &     11.7        & 34.0   & 54.0    & 36.7    & 31.2   & 51.0    & 32.7       \\
% PoolFormer-S12            &     12.0          & 37.3   & 59.0    & 40.1    & 34.6   & 55.8    & 36.9        \\
% EfficientFormer-L1        &     12.3              & 37.9   & 60.3    & 41.0    & 35.4   & 57.3    & 37.3       \\
% EfficientFormerV2-S2      &     12.6              &  38.9  &  60.3   & 42.4  &    35.5    &   57.2      &  37.8      \\
% \rowcolor[gray]{0.92}
% EfficientFormerV2-S2\dagger     &     12.6              &  43.4  &  65.4   & 47.5  &    39.5    &   62.4      &  42.2      \\
% \hline
% ResNet50                  &      25.5           & 38.0   & 58.6    & 41.4    & 34.4   & 55.1    & 36.7      \\
% PoolFormer-S24            &     21.0            & 40.1   & 62.2    & 43.4    & 37.0   & 59.1    & 39.6     \\
% Swin-T                    &     29.0              & 42.2   & 64.4    & 46.2    & 39.1   & 64.6    & 42.0      \\
% % PVTv2-B2                  &                         & 45.3   & 67.1    & 49.6    & 41.2   & 64.2    & 44.4    \\
% % Twins-SVT-S               &                         & 43.4   & 66.0    & 47.3    & 40.3   & 63.2    & 43.4      \\
% EfficientFormer-L3        &         31.3     & 41.4   & 63.9    & 44.7    & 38.1   & 61.0    & 40.4      \\
% % CSwin-T                   &                         & 46.7   & 68.6    & 51.3    & 42.2   & 65.6    & 45.4     \\
% EfficientFormerV2-L       &       26.1      & 42.4   &  64.2  &  46.7   &  38.7   &  61.1   & 41.6           \\
% \rowcolor[gray]{0.92}
% EfficientFormerV2-L\dagger      &       26.1      & 44.7   &  66.3  &  48.8   &  40.4   &  63.5   & 43.2           \\
% \bottomrule
% \end{tabular}

\begin{tabular}{c|c|cccccc|c}
\toprule
\multirow{2}{*}{Backbone} & \multirow{2}{*}{Params (M)} & \multicolumn{6}{c}{Detection \& Instance Segmentation} & \multicolumn{1}{c}{Semantic}  \\ \cline{3-9}
                          &                         & AP$^{box}$    & AP$^{box}_{50}$   & AP$^{box}_{75}$   & AP$^{mask}$    & AP$^{mask}_{50}$   & AP$^{mask}_{75}$   & mIoU   \\
                          \hline
                          \hline
ResNet18                  &     11.7        & 34.0   & 54.0    & 36.7    & 31.2   & 51.0    & 32.7   & 32.9   \\
PoolFormer-S12            &     12.0          & 37.3   & 59.0    & 40.1    & 34.6   & 55.8    & 36.9     & 37.2  \\
EfficientFormer-L1        &     12.3              & 37.9   & 60.3    & 41.0    & 35.4   & 57.3    & 37.3   &  38.9  \\
% EfficientFormerV2-S2      &     12.6              &  38.9  &  60.3   & 42.4  &    35.5    &   57.2      &  37.8   &   \\
\rowcolor[gray]{0.92}
EfficientFormerV2-S2     &     12.6              &  43.4  &  65.4   & 47.5  &    39.5    &   62.4      &  42.2   & 42.4  \\
\hline
ResNet50                  &      25.5           & 38.0   & 58.6    & 41.4    & 34.4   & 55.1    & 36.7  &  36.7  \\
PoolFormer-S24            &     21.0            & 40.1   & 62.2    & 43.4    & 37.0   & 59.1    & 39.6  &  40.3 \\
Swin-T                    &     29.0              & 42.2   & 64.4    & 46.2    & 39.1   & 64.6    & 42.0   & 41.5  \\
% PVTv2-B2                  &                         & 45.3   & 67.1    & 49.6    & 41.2   & 64.2    & 44.4    \\
% Twins-SVT-S               &                         & 43.4   & 66.0    & 47.3    & 40.3   & 63.2    & 43.4      \\
EfficientFormer-L3        &         31.3     & 41.4   & 63.9    & 44.7    & 38.1   & 61.0    & 40.4   &  43.5 \\
% CSwin-T                   &                         & 46.7   & 68.6    & 51.3    & 42.2   & 65.6    & 45.4     \\
% EfficientFormerV2-L       &       26.1      & 42.4   &  64.2  &  46.7   &  38.7   &  61.1   & 41.6    &       \\
\rowcolor[gray]{0.92}
EfficientFormerV2-L      &       26.1      & 44.7   &  66.3  &  48.8   &  40.4   &  63.5   & 43.2     &   45.2   \\
\bottomrule
\end{tabular}

% }
\label{tab:coco_improved}
\end{table*}

% \begin{table}[]
% \centering
% % \small
% \caption{\textbf{Semantic segmentation} on ADE20K. EfficientFormerV2 models are integrated as feature encoder in Semantic FPN. \dagger~refers to the results obtained from the enhanced training recipe. }
% \begin{tabular}{c|c|c}
% \toprule
% Backbone             & Params (M) & mIoU \\
% \hline
% ResNet18             & 11.7 & 32.9 \\
% PoolFormer-S12       & 12.0 & 37.2 \\
% EfficientFormer-L1   & 12.3 & 38.9 \\
% EfficientFormerV2-S2 & 12.6 & 39.5 \\
% \rowcolor[gray]{0.92}
% EfficientFormerV2-S2\dagger & 12.6 & 42.4 \\
% \hline
% ResNet50             & 25.5 & 36.7 \\
% PoolFormer-S24       & 21.0 & 40.3 \\
% EfficientFormer-L3   & 31.3 & 43.5 \\
% % EfficientFormerV2-L & 26.1 & 39.7 \\
% \rowcolor[gray]{0.92}
% EfficientFormerV2-L\dagger & 26.1 & 45.2 \\
% \bottomrule
% \end{tabular}
% \label{tab:ade20k_improved}
% \end{table}

==> figs/mes.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/mes.pdf}  
    \caption{\textbf{\texttt{MES} \emph{vs.} Accuracy.} EfficientFormerV2 shows superior \texttt{MES} and accuracy on ImageNet-1K compared to existing work. \texttt{MES} is plotted in logarithmic scale.}
    \label{fig:mes}
\end{figure}



==> iccv2023AuthorKit/backup/supp_2_downstream.tex <==
\begin{table*}[]
\centering
% \small
\caption{
\textbf{Object detection \&
instance segmentation} on MS COCO 2017. We benchmark on Mask RCNN pipeline. \dagger~refers to the results obtained from the enhanced training recipe. }
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{c|c|cccccc}
% \toprule
% \multirow{2}{*}{Backbone} & \multirow{2}{*}{Params (M)} & \multicolumn{6}{c}{Detection \& Instance Segmentation}  \\ \cline{3-8}
%                           &                         & AP$^{box}$    & AP$^{box}_{50}$   & AP$^{box}_{75}$   & AP$^{mask}$    & AP$^{mask}_{50}$   & AP$^{mask}_{75}$      \\
%                           \hline
%                           \hline
% ResNet18                  &     11.7        & 34.0   & 54.0    & 36.7    & 31.2   & 51.0    & 32.7       \\
% PoolFormer-S12            &     12.0          & 37.3   & 59.0    & 40.1    & 34.6   & 55.8    & 36.9        \\
% EfficientFormer-L1        &     12.3              & 37.9   & 60.3    & 41.0    & 35.4   & 57.3    & 37.3       \\
% EfficientFormerV2-S2      &     12.6              &  38.9  &  60.3   & 42.4  &    35.5    &   57.2      &  37.8      \\
% \rowcolor[gray]{0.92}
% EfficientFormerV2-S2\dagger     &     12.6              &  43.4  &  65.4   & 47.5  &    39.5    &   62.4      &  42.2      \\
% \hline
% ResNet50                  &      25.5           & 38.0   & 58.6    & 41.4    & 34.4   & 55.1    & 36.7      \\
% PoolFormer-S24            &     21.0            & 40.1   & 62.2    & 43.4    & 37.0   & 59.1    & 39.6     \\
% Swin-T                    &     29.0              & 42.2   & 64.4    & 46.2    & 39.1   & 64.6    & 42.0      \\
% % PVTv2-B2                  &                         & 45.3   & 67.1    & 49.6    & 41.2   & 64.2    & 44.4    \\
% % Twins-SVT-S               &                         & 43.4   & 66.0    & 47.3    & 40.3   & 63.2    & 43.4      \\
% EfficientFormer-L3        &         31.3     & 41.4   & 63.9    & 44.7    & 38.1   & 61.0    & 40.4      \\
% % CSwin-T                   &                         & 46.7   & 68.6    & 51.3    & 42.2   & 65.6    & 45.4     \\
% EfficientFormerV2-L       &       26.1      & 42.4   &  64.2  &  46.7   &  38.7   &  61.1   & 41.6           \\
% \rowcolor[gray]{0.92}
% EfficientFormerV2-L\dagger      &       26.1      & 44.7   &  66.3  &  48.8   &  40.4   &  63.5   & 43.2           \\
% \bottomrule
% \end{tabular}

\begin{tabular}{c|c|cccccc|c}
\toprule
\multirow{2}{*}{Backbone} & \multirow{2}{*}{Params (M)} & \multicolumn{6}{c}{Detection \& Instance Segmentation} & \multicolumn{1}{c}{Semantic}  \\ \cline{3-9}
                          &                         & AP$^{box}$    & AP$^{box}_{50}$   & AP$^{box}_{75}$   & AP$^{mask}$    & AP$^{mask}_{50}$   & AP$^{mask}_{75}$   & mIoU   \\
                          \hline
                          \hline
ResNet18                  &     11.7        & 34.0   & 54.0    & 36.7    & 31.2   & 51.0    & 32.7   & 32.9   \\
PoolFormer-S12            &     12.0          & 37.3   & 59.0    & 40.1    & 34.6   & 55.8    & 36.9     & 37.2  \\
EfficientFormer-L1        &     12.3              & 37.9   & 60.3    & 41.0    & 35.4   & 57.3    & 37.3   &  38.9  \\
% EfficientFormerV2-S2      &     12.6              &  38.9  &  60.3   & 42.4  &    35.5    &   57.2      &  37.8   &   \\
\rowcolor[gray]{0.92}
EfficientFormerV2-S2     &     12.6              &  43.4  &  65.4   & 47.5  &    39.5    &   62.4      &  42.2   & 42.4  \\
\hline
ResNet50                  &      25.5           & 38.0   & 58.6    & 41.4    & 34.4   & 55.1    & 36.7  &  36.7  \\
PoolFormer-S24            &     21.0            & 40.1   & 62.2    & 43.4    & 37.0   & 59.1    & 39.6  &  40.3 \\
Swin-T                    &     29.0              & 42.2   & 64.4    & 46.2    & 39.1   & 64.6    & 42.0   & 41.5  \\
% PVTv2-B2                  &                         & 45.3   & 67.1    & 49.6    & 41.2   & 64.2    & 44.4    \\
% Twins-SVT-S               &                         & 43.4   & 66.0    & 47.3    & 40.3   & 63.2    & 43.4      \\
EfficientFormer-L3        &         31.3     & 41.4   & 63.9    & 44.7    & 38.1   & 61.0    & 40.4   &  43.5 \\
% CSwin-T                   &                         & 46.7   & 68.6    & 51.3    & 42.2   & 65.6    & 45.4     \\
% EfficientFormerV2-L       &       26.1      & 42.4   &  64.2  &  46.7   &  38.7   &  61.1   & 41.6    &       \\
\rowcolor[gray]{0.92}
EfficientFormerV2-L      &       26.1      & 44.7   &  66.3  &  48.8   &  40.4   &  63.5   & 43.2     &   45.2   \\
\bottomrule
\end{tabular}

% }
\label{tab:coco_improved}
\end{table*}

% \begin{table}[]
% \centering
% % \small
% \caption{\textbf{Semantic segmentation} on ADE20K. EfficientFormerV2 models are integrated as feature encoder in Semantic FPN. \dagger~refers to the results obtained from the enhanced training recipe. }
% \begin{tabular}{c|c|c}
% \toprule
% Backbone             & Params (M) & mIoU \\
% \hline
% ResNet18             & 11.7 & 32.9 \\
% PoolFormer-S12       & 12.0 & 37.2 \\
% EfficientFormer-L1   & 12.3 & 38.9 \\
% EfficientFormerV2-S2 & 12.6 & 39.5 \\
% \rowcolor[gray]{0.92}
% EfficientFormerV2-S2\dagger & 12.6 & 42.4 \\
% \hline
% ResNet50             & 25.5 & 36.7 \\
% PoolFormer-S24       & 21.0 & 40.3 \\
% EfficientFormer-L3   & 31.3 & 43.5 \\
% % EfficientFormerV2-L & 26.1 & 39.7 \\
% \rowcolor[gray]{0.92}
% EfficientFormerV2-L\dagger & 26.1 & 45.2 \\
% \bottomrule
% \end{tabular}
% \label{tab:ade20k_improved}
% \end{table}

==> iccv2023AuthorKit/figs/0_main.tex <==
\begin{figure*}[]
    \centering
    \includegraphics[width=1\linewidth]{figures/main.pdf}  
    \caption{\textbf{Network architectures.} We consider three metrics, \emph{i.e.}, model performance, size, and inference speed, and study the models that improve any metric without hurting others. (a) Network of EfficientFormer~\cite{efficientformer} that serves as a baseline model. (b) Unified FFN (Sec.~\ref{sec:mixer}). (c) MHSA improvements (Sec.~\ref{sec:improve_mhsa}). (d)\&(e) Attention on higher resolution (Sec.~\ref{sec:higher_res}). (f) Dual-Path Attention downsampling (Sec.~\ref{sec:subsample}).}
    \label{fig:main}
\end{figure*}

==> iccv2023AuthorKit/figs/comparison.tex <==
\begin{figure}[]
    \centering
    \includegraphics[width=1\linewidth]{figures/bubble.pdf}  
    \caption{\textbf{Comparison of model size, speed, and performance (top-1 accuracy on ImageNet-1K).}
    % Models are trained on ImageNet-1K to get top-1 accuracy.
    Latency is profiled by iPhone 12 (iOS 16). The area of each circle is proportional to the number of parameters (model size). EfficientFormerV2 achieves high performance with small model sizes and fast inference speed. }
    \label{fig:bubble}
\end{figure}

==> iccv2023AuthorKit/figs/mes.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/mes.pdf}  
    \caption{\textbf{\texttt{MES} \emph{vs.} Accuracy.} EfficientFormerV2 shows superior \texttt{MES} and accuracy on ImageNet-1K compared to existing work. \texttt{MES} is plotted in logarithmic scale.}
    \label{fig:mes}
\end{figure}



==> iccv2023AuthorKit/figs/more_random.tex <==
% \setlength{\intextsep}{1pt}%
% \setlength{\columnsep}{2pt}%
% \begin{wrapfigure}{r}{0.5\linewidth}
% % \vspace{-2em}
% \includegraphics[trim={1mm 0mm 1mm 8mm},clip,width=1\linewidth]{iccv2023AuthorKit/figures/random.pdf}
% %   \end{center}
%   \caption{Comparisons with more random sampled models. We take 0.1ms as the significant digit based on mobile measurement precision. }
% % \vspace{-7mm}
% \label{fig:more_random}
% \end{wrapfigure}
\begin{figure}
    \centering
\includegraphics[trim={1mm 0mm 1mm 8mm},clip,width=0.8\linewidth]{iccv2023AuthorKit/figures/random.pdf}
%   \end{center}
  \caption{Comparisons with more random sampled models. We take 0.1ms as the significant digit based on mobile measurement precision. }
% \vspace{-7mm}
\label{fig:more_random}
\end{figure}

==> iccv2023AuthorKit/figs/subnet_evaluation.tex <==
% \setlength{\intextsep}{1pt}%
% \setlength{\columnsep}{2pt}%
% \begin{wrapfigure}{r}{0.5\linewidth}
% \includegraphics[trim={1mm 0mm 1mm 6mm},clip,width=1\linewidth]{iccv2023AuthorKit/figures/cor.pdf}
% %   \end{center}
% % \captionof{figure}{Subnet evaluation vs. training from scratch. We report our searched models (red) along with random ones (blue). }
% % \vspace{-7mm}
% \end{wrapfigure}
\begin{figure}
    \centering
\includegraphics[trim={1mm 0mm 1mm 6mm},clip,width=0.8\linewidth]{iccv2023AuthorKit/figures/cor.pdf}
%   \end{center}
\caption{Subnet evaluation vs. training from scratch. We report our searched models (red) along with random ones (blue). }
    \label{fig:correlation}
\end{figure}

==> iccv2023AuthorKit/sections/0_abstract.tex <==
\begin{abstract}
With the success of Vision Transformers (ViTs) in computer vision tasks, recent arts try to optimize the performance and complexity of ViTs to enable efficient deployment on mobile devices.
Multiple approaches are proposed to accelerate attention mechanism, improve inefficient designs, or incorporate mobile-friendly lightweight convolutions to form hybrid architectures.
However, ViT and its variants still have \emph{higher latency} or considerably \emph{more parameters} than lightweight CNNs, even true for the years-old MobileNet. 
In practice, latency and size are both crucial for efficient deployment on resource-constraint hardware. 
In this work, we investigate a central question, can transformer models run as fast as MobileNet and maintain a similar size? 
We revisit the design choices of ViTs and propose a novel supernet with low latency and high parameter efficiency. 
We further introduce a novel fine-grained joint search strategy for transformer models that can find efficient architectures by optimizing latency and number of parameters simultaneously. The proposed models, EfficientFormerV2, achieve $3.5\%$ higher top-1 accuracy than MobileNetV2 on ImageNet-1K with similar latency and parameters. This work demonstrate that properly designed and optimized vision transformers can achieve high performance even with MobileNet-level size and speed.
% \footnote{Code: ~\href{https://github.com/snap-research/EfficientFormer}{\color{urlcolor}{https://github.com/snap-research/EfficientFormer}}.}



\end{abstract}



==> iccv2023AuthorKit/sections/1_intro.tex <==
\section{Introduction}

\input{figs/comparison}
The promising performance of Vision Transformers (ViTs)~\cite{dosovitskiy2020vit} has inspired many follow-up works to further refine the model architecture and improve training strategies, leading to superior results on most computer vision benchmarks, such as classification~\cite{liu2021swin2,liu2021video,caron2021emerging,ma2022multimodal}, segmentation~\cite{xie2021segformer,cheng2021masked,cai2022efficientvit}, detection~\cite{carion2020end,li2021improved,si2022inception}, and image synthesis~\cite{esser2021taming,han2022show}.
As the essence of ViT, Multi Head Self Attention (MHSA) mechanism is proved to be effective in modeling spatial dependencies in $2$D images, enabling a global receptive field. 
In addition, MHSA learns second-order information with the attention heatmap as dynamic weights, which is a missing property in Convolution Neural Networks (CNNs) \cite{han2021connection}.
However, the cost of MSHA is also obvious--quadratic computation complexity with respect to the number of tokens (resolution).
Consequently, ViTs tend to be more computation intensive and have higher latency compared to widely adopted lightweight CNNs~\cite{howard2017mobilenets,howard2019searching}, especially on resource-constrained mobile devices, limiting their wide deployment in real-world applications.

Many research efforts~\cite{mehta2021mobilevit,mehta2022separable, pan2022edgevits,efficientformer} are taken to alleviate this limitation. 
Among them, one direction is to reduce the quadratic computation complexity of the attention mechanism.
Swin \cite{liu2021swin} and following works~\cite{dong2022cswin,liu2021swin2} propose window-based attention such that the receptive field is constrained to a pre-defined window size, which also inspires subsequent work to refine attention patterns \cite{chen2021crossvit,wang2021crossformer,wu2022pale,pan2022fast}. 
With the pre-defined span of attention, the computation complexity becomes linear to resolution. 
However, sophisticated attention patterns are generally difficult to support or accelerate on mobile devices because of intensive shape and index operations. 
Another track is to combine lightweight CNN and attention mechanism to form a hybrid architecture \cite{mehta2021mobilevit,chen2021mobile,maaz2022edgenext}. 
The benefit comes two-fold. First, convolutions are shift invariant and are good at capturing local and detailed information, which can be considered as a good complement to ViTs \cite{han2021connection}. 
Second, by placing convolutions in the early stages while placing MHSA in the last several stages to model global dependency, we can naturally avoid performing MHSA on high resolution and save computations \cite{liu2022uninet}. 
Albeit achieving satisfactory performance, the latency and model size are still less competitive compared to lightweight CNNs. 
For instance, MobileViT~\cite{mehta2021mobilevit} achieves better performance than MobileNetV2 while being at least $5\times$ slower on iPhone 12. 
As applicable to CNNs, architecture search, pruning, and quantization techniques are also thoroughly investigated \cite{jin2021teachers,jin2022f8net,liu2021post,kim2021bert,chavan2022vision,efficientformer,liu2022uninet}. 
Nevertheless, these models still emerge obvious weaknesses,   
\emph{e.g.}, EfficientFormer-L1~\cite{efficientformer} achieves comparable speed and better performance than MobileNetV2$\times1.4$, while being $2\times$ larger. 
Thus, a \emph{practical} yet \emph{challenging} question arises:

\emph{Can we design a transformer-based model that is both light and fast, and preserves high performance}?



In this work, we address the above question and propose a new family of mobile vision backbones. 
We consider three vital factors: \emph{number of parameters}, \emph{latency}, and \emph{model performance}, as they reflect disk storage and mobile applications.
First, we introduce \emph{novel architectural improvements} to form a strong design paradigm.  
Second, we propose a \emph{fine-grained} architecture search algorithm that jointly optimizes model size and speed for transformer models. 
With our network design and search method, we obtain a series of models under various constraints of model size and speed while maintaining high performance, named EfficientFormerV2. 
Under the exact same size and latency (on iPhone 12), EfficientFormerV2-S0 outperforms MobileNetV2 by $3.5\%$ higher top-1 accuracy on ImageNet-1K~\cite{deng2009imagenet}.
Compared to EfficientFormer-L1~\cite{efficientformer}, EfficientFormerV2-S1 has similar performance while being $2\times$ smaller and $1.3\times$ faster (Tab.~\ref{tab:comparison}). 
We further demonstrate promising results in downstream tasks such as detection and segmentation (Tab.~\ref{tab:coco}).
% We hope our work can shed light on the study of small-size, fast-speed, and high-performance mobile ViT models.
Our contributions can be concluded as follows.
\begin{itemize}[leftmargin=1em]
\setlength
\itemsep{-0.25em}
    \item We comprehensively study mobile-friendly design choices and introduce novel changes, which is a practical guide to obtaining ultra-efficient vision transformer backbones.
    \item We propose a novel fine-grained joint search algorithm that simultaneously optimizes model size and speed for transformer models, achieving superior Pareto optimality.
    \item For the first time, we show that vision transformer models can be as small and fast as MobileNetV2 while obtaining much better performance. EfficientFormerV2 can serve as a strong backbone in various downstream tasks.
    % achieves ultra-fast inference and ultra-tiny model size, 
    % outperforming previous arts by a large margin, and can serve as a strong backbone in various downstream tasks. 
\end{itemize}



% focus on efficient transformer models that can be deployed on mobile devices~\cite{mehta2021mobilevit,efficientformer,pan2022edgevits}. They primarily  Yet the joint improvement of these factors remains a challenge. Existing work shows that, although lightweight CNNs, \emph{e.g.}, MobileNetV2~\cite{sandler2018mobilenetv2}, have inferior model performance than efficient ViTs, they still hold clear advantages over the number of parameters or the latency.  
% Firstly, we revisit recent arts on efficient ViT and provide a comprehensive analysis. 
% We ...
% Secondly, we propose a joint metric to optimize size and speed simultaneously. 
% We ...
% Our contribution can be concluded as follows, 

% which can be categorized into there main tracks. The \emph{first} promising direction focuses on finding efficient attention to achieve around linear computation complexity, such as window-based attention~\cite{liu2021swin,dong2022cswin} and kernel-based attention~\cite{}. However, the window-based attention requiring sophisticated attention patterns, which are generally hard to accelerate on mobile devices due to intensive shape and index operations~\cite{}, and kernel-based attention shows inferior performance than Softmax attention~\cite{}. The \emph{second} track targets on combining lightweight CNN and ViT to form a hybird architecture~\cite{} to leverage efficient convolution for capturing local information~\cite{}. Albeit reducing model size and obtaining satisfactory performance, the latency is much slower than CNNs~\cite{}. The \emph{third} one leverages the compression techniques from CNNs~\cite{} to find a latency friendly architecture~\cite{}. Nevertheless, these models contains more parameters than CNNs, requiring more disk storage for running them on devices

% After carefully reviewing existing works, two major challenges remain for mobile-friendly ViTs. \emph{First}, it mains unclear what are the most mobile-friendly design for vision transformer, even though extensively investigated. Additionally, a large portion of network optimizations are not mobile friendly~\cite{liu2021swin}. As a result, for the architecture level, the effectiveness of network optimization approaches, \emph{e.g.}, complexity reduction, require careful verification.
% \emph{Second}, number of parameters and latency are the two vital metrics for evaluating an on-device model, while most existing works solely target optimizing one of them for ViTs. Thus, under similar model performance, light-weight CNNs such as MobileNetV2~\cite{}, still holds clear advantages over efficient ViTs. 
% we notice an interesting phenomenon that recent research solely focus on optimizing one metric, i.e., size (parameters) \cite{}, or FLOPs \cite{}, or speed \cite{}. However, this easily enters a pitfall that the optimized performance on one metric is achieved by sacrificing another. 
% For instance, size-oriented backbone MobileViT~\cite{mehta2021mobilevit} achieves comparable or better performance than MobileNetV2 at the cost of being least $5\times$ slower on iPhone 12, and EfficientFormer~\cite{} achieves comparable speed and better performance than MobileNetV2 while has the network size times larger than MobileNetV2. 
% In general, size and speed are both important constraints for mobile deployment.
% Thus, an interesting yet challenging question arises, \emph{can we design a transformer-based model that is light, fast, and high-performance}? 


% Among them, a promising track is to enable efficient attention with linear complexity. 
% Swin \cite{liu2021swin} and the following works~\cite{dong2022cswin} propose window-based attention such that the receptive field is constrained to a predefined window size, which also inspires subsequent work to refine attention patterns \cite{}. 
% With the predefined span of attention, the computation complexity becomes linear to input number of tokens (resolution). 
% However, sophisticated attention patterns are generally difficult to support or accelerate on mobile device \cite{} because of intensive shape and index operations. 
% Kernel-based attention \cite{} refine the SoftMax computation in MHSA to kernel-based similarity, which is commutative to matrix multiplication. 
% As a result, the dot product of keys and values can be pre-computed, enables a linear complexity in token dimension. 
% But kernel-based attention only shows significant speedup under high resolution \cite{}, which restricts its benefits in mobile scenario, and the performance can be inferior to SoftMax attention \cite{}. 

% Another track is to combine lightweight CNN and ViT to form a hybrid architecture \cite{}. 
% The benefit comes two-fold. First, convolutions
% are shift invariant and are good at capturing local and detail information, which can be considered as a good complement to ViTs \cite{}. 
% Second, by placing convolutions in early stages while placing MHSA in last several stages to model global dependency, we can naturally avoid performing MHSA on high resolution and save computations \cite{}. 
% MobileViT \cite{} and MobileFormer \cite{} integrate MobileNet block into ViT backbone to reduce model size, but the latency is still not satisfactory compared to SOTA CNNs \cite{}. 

% Moreover, as also applicable to CNNs, network pruning \cite{}, search \cite{}, and quantization \cite{} have been investigated to generate efficient ViTs. 
% It is notable that recent work EfficientFormer \cite{} leverage latency-driven search to generate fast and accurate networks, but the architecture requires considerable amount of parameters, which enlarges model size and limits its deployment on mobile devices. 



% \textbf{problem}
% Inspired by these observations, we conclude two major challenges for mobile-friendly ViTs. 
% (i) Though extensively investigated, it remains unclear which is the most mobile-suitable design for vision transformer, and a large portion of optimizations \cite{liu2021swin} are not mobile favorable. 
% As a result, at design level, the effectiveness of architecture optimization methods (i.e. complexity reduction, convolution injection) require careful verification. 
% (ii) We notice an interesting phenomenon that recent research solely focus on optimizing one metric, i.e., size (parameters) \cite{}, or FLOPs \cite{}, or speed \cite{}. However, this easily enters a pitfall that the optimized performance on one metric is achieved by sacrificing another. 
% For instance, size-oriented backbone MobileViT \cite{mehta2021mobilevit} achieves comparable or better performance than traditional lightweight CNNs \cite{}, but the speed is at least $5\times$ slower on iPhone. 
% In contrast, LeViT \cite{} and EfficientFormer \cite{} achieves FLOPs and speed SOTA respectively, but the network size is times larger than lightweight CNNs. 
% In general, size and speed are both important constraints for mobile deployment.
% Thus, a central question arises, \emph{can we construct a vision backbone that is both light and fast}? 




% ===============V1==========================
% Vision Transformer (ViT)~\cite{dosovitskiy2020vit} and its variants \cite{} have achieved state-of-the-art performance in most popular vision tasks, including classification~\cite{}, segmentation~\cite{}, detection~\cite{}, etc. 
% As the essence of ViT, Multi Head Self Attention (MHSA) mechanism is proved to be effective in modeling spatial dependencies in 2D image, enabling a global receptive field. 
% In addition, MHSA learns second order information with the attention heatmap as dynamic weights, which is a missing property in traditional Convolution Neural Networks (CNNs). 
% On the downside, these properties are achieved at the cost of quadratic computation complexity with respect to image patches, i.e., resolution. 
% Consequently, ViTs tend to be computation intensive and speed disadvantageous \cite{} compared to popular lightweight CNNs \cite{}, especially on mobile devices \cite{} which is the scope of this work. 

% Efficient deployment of ViT has emerged lots of research interests \cite{}. 
% Among them, a promising track is to enable efficient attention with linear complexity. 
% Swin \cite{liu2021swin} propose window-based attention such that the receptive field is constrained to a predefined window size, which also inspires subsequent work to refine attention patterns \cite{}. 
% With the predefined span of attention, the computation complexity becomes linear to input number of tokens (resolution). 
% However, sophisticated attention patterns are generally difficult to support or accelerate on mobile device \cite{} because of intensive shape and index operations. 
% Kernel-based attention \cite{} refine the SoftMax computation in MHSA to kernel-based similarity, which is commutative to matrix multiplication. 
% As a result, the dot product of keys and values can be pre-computed, enables a linear complexity in token dimension. 
% But kernel-based attention only shows significant speedup under high resolution \cite{}, which restricts its benefits in mobile scenario, and the performance can be inferior to SoftMax attention \cite{}. 

% Another track is to combine lightweight CNN and ViT to form a hybrid architecture \cite{}. 
% The benefit comes two-fold. First, convolutions
% are shift invariant and are good at capturing local and detail information, which can be considered as a good complement to ViTs \cite{}. 
% Second, by placing convolutions in early stages while placing MHSA in last several stages to model global dependency, we can naturally avoid performing MHSA on high resolution and save computations \cite{}. 
% MobileViT \cite{} and MobileFormer \cite{} integrate MobileNet block into ViT backbone to reduce model size, but the latency is still not satisfactory compared to SOTA CNNs \cite{}. 

% Moreover, as also applicable to CNNs, network pruning \cite{}, search \cite{}, and quantization \cite{} have been investigated to generate efficient ViTs. 
% It is notable that recent work EfficientFormer \cite{} leverage latency-driven search to generate fast and accurate networks, but the architecture requires considerable amount of parameters, which enlarges model size and limits its deployment on mobile devices. 


% \textbf{problem}
% Inspired by these observations, we conclude two major challenges for mobile-friendly ViTs. 
% (i) Though extensively investigated, it remains unclear which is the most mobile-suitable design for vision transformer, and a large portion of optimizations \cite{liu2021swin} are not mobile favorable. 
% As a result, at design level, the effectiveness of architecture optimization methods (i.e. complexity reduction, convolution injection) require careful verification. 
% (ii) We notice an interesting phenomenon that recent research solely focus on optimizing one metric, i.e., size (parameters) \cite{}, or FLOPs \cite{}, or speed \cite{}. However, this easily enters a pitfall that the optimized performance on one metric is achieved by sacrificing another. 
% For instance, size-oriented backbone MobileViT \cite{mehta2021mobilevit} achieves comparable or better performance than traditional lightweight CNNs \cite{}, but the speed is at least $5\times$ slower on iPhone. 
% In contrast, LeViT \cite{} and EfficientFormer \cite{} achieves FLOPs and speed SOTA respectively, but the network size is times larger than lightweight CNNs. 
% In general, size and speed are both important constraints for mobile deployment.
% Thus, a central question arises, \emph{can we construct a vision backbone that is both light and fast}? 


% \textbf{our solution and contribution}
% In this work, we address these challenges and propose a mobile-friendly vision backbone. 
% Firstly, we revisit recent arts on efficient ViT and provide a comprehensive analysis. 
% We ...
% Secondly, we propose a joint metric to optimize size and speed simultaneously. 
% We ...
% Our contribution can be concluded as follows, 





==> iccv2023AuthorKit/sections/2_related_work.tex <==
\section{Related Work}
% \textcolor{red}{Add references for deformable attention, hydra attention}
Vaswani \textit{et al.}~\cite{vaswani2017attention} propose attention mechanism to model sequences in NLP task, which forms transformer architecture. 
Transformers are later adopted to vision tasks by Dosovitskiy \textit{et al.}~\cite{dosovitskiy2020vit} and Carion~\textit{et al.}~\cite{carion2020end}. 
DeiT~\cite{touvron2021training} improves ViT by training with distillation and achieves competitive performance against CNNs. 
Later research further improves ViTs by incorporating hierarchical design~\cite{wang2021pyramid,touvron2021going}, injecting locality with the aid of convolutions~\cite{guo2021cmt,dai2021coatnet,han2021connection,si2022inception}, or exploring different types of token mixing such as local attention~\cite{liu2021swin,dong2022cswin}, spatial MLP mixer~\cite{touvron2021resmlp,tolstikhin2021mixer}, and non-parameterized pool mixer~\cite{yu2021metaformer}. 
With appropriate changes, ViTs demonstrate strong performance in downstream vision tasks~\cite{xie2021segformer,zhang2022nested,zhang2022topformer,lee2021vision,lee2021vitgan,esser2021taming,zeng2021improving}. 
To benefit from the advantageous performance, efficient deployment of ViTs has become a research hotspot, especially for mobile devices~\cite{mehta2021mobilevit,chen2021mobile,pan2022edgevits,maaz2022edgenext}.
For reducing the computation complexity of ViTs,  
many works propose new modules and architecture design~\cite{Nikita2020,hassani2021escaping,fayyaz2021ats,Wei2022,Renggli2022}, while others eliminate redundancies in attention mechanism~\cite{wang2021crossformer,heo2021rethinking,chen2021regionvit,li2021localvit,chu2021twins,rao2021dynamicvit,Zhengzhong2022,hydraattention}. 
Similar to CNNs, architecture search~\cite{chen2021autoformer,gong2022nasvit,chavan2022vision,zhou2022training,liu2022uninet,fbnetv3,fbnetv5}, pruning~\cite{zhang2022platon}, and quantization~\cite{liu2021post} are also explored for ViTs. 

We conclude two major drawbacks of the study in efficient ViT.
First, many optimizations are not suitable for mobile deployment. For example, the quadratic computation complexity of the attention mechanism can be reduced to linear by regularizing the span or pattern of attention mechanism~\cite{liu2021swin,dong2022cswin,chen2021crossvit,deformableattention}. Still, the sophisticated reshaping and indexing operations are not even supported on resource-constrained devices~\cite{efficientformer}. 
It is crucial to rethink the mobile-friendly designs. 
Second, though recent hybrid designs and network search methods reveal efficient ViTs with strong performance~\cite{mehta2021mobilevit,liu2022uninet,efficientformer}, they mainly optimize the Pareto cure for one metric while being less competitive in others. 
For example, MobileViT~\cite{mehta2021mobilevit} is parameter efficient while being times slower than lightweight CNNs~\cite{sandler2018mobilenetv2,tan2019efficientnet}. 
EfficientFormer~\cite{efficientformer} wields ultra-fast speed on mobile, but the model size is enormous. 
LeViT~\cite{levit} and MobileFormer~\cite{chen2021mobile} achieve favorable FLOPs at the cost of redundant parameters. 

% \textcolor{blue}{
% Transformers are initially proposed to handle the learning of long sequences in NLP tasks~\cite{vaswani2017attention}. 
% Dosovitskiy \textit{et al.}~\cite{dosovitskiy2020vit} and Carion \textit{et al.}~\cite{carion2020end} adapt the transformer architecture to classification and detection, respectively, and achieve competitive performance against CNN counterparts with stronger training techniques and larger-scale datasets. 
% DeiT~\cite{touvron2021training} further improves the training pipeline with the aid of distillation, eliminating the need for large-scale pretraining~\cite{yuan2021tokens}. 
% Inspired by the competitive performance and global receptive field of transformer models, follow-up works are proposed to refine the architecture~\cite{wang2021pyramid,touvron2021going}, explore the relationship between CONV nets and ViT~\cite{guo2021cmt,dai2021coatnet,han2021connection}, and adapt ViT to different computer vision tasks~\cite{xie2021segformer,zhang2022nested,zhang2022topformer,lee2021vision,lee2021vitgan,esser2021taming,zeng2021improving}. Other research efforts explore the essence of attention mechanism and propose insightful variants of token mixer, \textit{e.g.}, local attention~\cite{liu2021swin}, spatial MLP~\cite{touvron2021resmlp,tolstikhin2021mixer}, and pooling-mixer~\cite{yu2021metaformer}. 
% Despite the success in most vision tasks, ViT-based models cannot compete with the well-studied lightweight CNNs \cite{sandler2018mobilenetv2,tan2019efficientnet} when the inference speed is the major concern~\cite{tolstikhin2021mlp,chen2021cyclemlp,zhou2021deepvit}, especially on resource-constrained edge devices \cite{wang2022towards}. 
% To accelerate ViT, many approaches have been introduced with different methodologies, such as proposing new architectures or modules~\cite{Nikita2020,chen2021crossvit,hassani2021escaping,fayyaz2021ats,Wei2022,Renggli2022}, re-thinking self-attention and sparse-attention mechanisms~\cite{wang2021crossformer,heo2021rethinking,chen2021regionvit,li2021localvit,chu2021twins,rao2021dynamicvit,Zhengzhong2022}, 
% and utilizing search algorithms that are widely explored in CNNs to find smaller and faster ViTs~\cite{chen2021autoformer,gong2022nasvit,chavan2022vision,zhou2022training}. 
% Recently, LeViT~\cite{Graham_2021_ICCV} proposes a CONV-clothing design to accelerate vision transformer. However, in order to perform MHSA, the $4$D features need to be frequently reshaped into flat patches, which is still expensive to compute on edge resources (Fig.~\ref{fig:speed}). Likewise, MobileViT~\cite{mehta2021mobilevit} introduces a hybrid architecture that combines lightweight MobileNet blocks (with point-wise and depth-wise CONV) and MHSA blocks; the former is placed at early stages in the network pipeline to extract low-level features, while the latter is placed in late stages to enjoy the global receptive field. 
% Similar approach has been explored by several works~\cite{chen2021mobile,gong2022nasvit} as a straightforward strategy to reduce computation.
% Different from existing works, we aim at pushing the latency-performance boundary of pure vision transformers instead of relying on hybrid designs, and directly optimize for mobile latency. Through our detailed analysis (Sec.~\ref{sec:latency}), we propose a new design paradigm (Sec.~\ref{sec:network_design}), which can be further elevated through architecture search (Sec.~\ref{sec:search}). 
% }

==> iccv2023AuthorKit/sections/3_method.tex <==
\section{Rethinking Hybrid Transformer Network} \label{sec:3rethink}

\input{figs/0_main}

% To the best of our knowledge, this work is the first attempt to jointly optimize model size and speed, and as will be shown later, significant improvements can be achieved compared to current SOTA vision backbones which are designed and optimized with single constraint. 

% ============== V1 ============== 
% As discussed, optimizing the Pareto curve merely on one metric easily enters a pitfall that the good performance is achieved by sacrificing too much on another. 
% Before we dive into architecture designs and performance analysis, we need a unified and fair metric to assess the network. 
% Without loss of generality, we define a \underline{m}obile \underline{e}fficiency \underline{score} (\texttt{meScore}) as follows,
% \begin{equation}
%     \texttt{meScore} = \texttt{S} \cdot \prod_i (\frac{M_i}{U_i})^{-1}
% \end{equation}
% Where \texttt{S} is a predefined base score (i.e. 100), $i \in \{$size, latency, memory footprint, energy consumption, ...$\}$, $M_i$ and $U_i$ are the corresponding metric and its unit. 
% For simplicity in this work, we only discuss model size and speed. 
% Size is determined by the number of parameters stored in the model, while speed depends on computation complexity (MACs) and hardware. 
% Since we focus on mobile deployment, we take the size and speed of MobileNetV2 as a score baseline. 
% Specifically, we define $U_{size}$ as 3M parameters, and $U_{latency}$ as 1ms inference latency on iPhone 12 deployed with CoreMLTools. 
% Intuitively, a model with 3M parameters and 1ms inference latency obtains a \texttt{meScore} of 100, while \texttt{meScore} drops to 25 on a larger model with doubled parameters (6M) and latency (2ms). 
% We believe the form of \texttt{meScore} is general and can possibly inspire future research by extending to other metrics of interest, such as inference-time memory footprint, energy consumption, etc. Plus, the importance (slope) of each metric is easily adjustable by appropriately defining $U_i$. 
% To the best of our knowledge, this work is the first attempt to jointly optimize model size and speed, and as will be shown later, significant improvements can be achieved compared to current SOTA vision backbones which are designed and optimized with single constraint. 

% \subsection{Rethinking Hybrid Transformer Architecture}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\input{tabs/0_analysis}

In this section, we study the design choices for efficient ViTs and introduce the changes that lead to the smaller size and faster speed without a performance drop.  EfficientFormer-L1~\cite{efficientformer} is used as a baseline model given its superior performance on mobile devices. 

\subsection{Token Mixers \emph{vs.} Feed Forward Network}\label{sec:mixer}
Incorporating local information can improve performance and make ViTs more robust to the absence of explicit positional embedding~\cite{cai2022efficientvit}. 
PoolFormer~\cite{yu2021metaformer} and EfficientFormer~\cite{efficientformer} employ $3\times3$ average pooling layers (Fig.~\ref{fig:main}{(a)}) as local token mixer. Replacing these layers with depth-wise convolutions (DWCONV) of the same kernel size does not introduce latency overhead, while the performance is improved by $0.6\%$ with negligible extra parameters ($0.02$M).
Further, recent work \cite{gong2022nasvit,cai2022efficientvit} suggest that it is also beneficial to inject local information modeling layers in the Feed Forward Network (FFN) in ViTs to boost performance with minor overhead. 
It is noteworthy that by placing extra depth wise $3\times 3$ convolutions in FFNs to capture local information, the functionality of original local mixer (pooling or convolution) is duplicated.
Based on these observations, we remove the explicit residual-connected local token mixer and move the dept-wise $3\times3$ CONV into the FFN, to get a unified FFN (Fig.~\ref{fig:main}{(b)}) with locality enabled. 
We apply the unified FFN to all stages of the network, as in Fig.~\ref{fig:main}{(a,b)}. 
Such design modification simplifies the network architecture to only two types of blocks (local FFN and global attention), and boosts the accuracy to $80.3\%$ at the same latency (see Tab.~\ref{tab:rethink_design}) with minor overhead in parameters ($0.1$M). 
More importantly, this modification allows us to \emph{directly search the network depth} with the exact number of modules in order to extract local and global information, 
especially at the late stages of the network, as discussed in Sec.~\ref{sec:joint_search}.


% ====================== V1% ====================== 
% \subsection{Unify Local Mixer and Feed Forward Block}\label{sec:mixer}
% In PoolFormer \cite{yu2021metaformer} and EfficientFormer \cite{}, local mixers are set as $3\times 3$ average pooling for simplicity. 
% In fact, there is no computation overhead to parameterize pooling layers to depth wise convolutions with same kernel size. 
% As in Tab.~\ref{tab:analysis}, we observe $0.6\%$ performance improvement by simply changing $3\times 3$ pooling to depth wise convolutions, and the extra parameters ($0.02$M) are negligible. 

% Further, recent work \cite{} find that it is beneficial to inject local information modeling layers in the Feed Forward Network (FFN) in ViTs to improve performance with minor overhead. 
% With the additional local information, ViTs prone to be more robust to the absence of explicit position embedding as well \cite{}. 
% It is noteworthy that by placing extra depth wise $3\times 3$ convolutions in FFNs to capture local information, the functionality of original local mixer (pooling or convolution) is duplicated.
% Since we are able to determine the desired number of local mixers by searching the depth in the final step, we delete the original residual-connected mixer and propose a unified FFN with local token mixing enabled for both local and global stages of the network, as shown in Fig.~\ref{fig:main}\todo{(b)}. 
% With this design refinement, we boost the accuracy to 80.3\% with minor overhead in parameters (0.1M), and the latency remains unchanged. 

\subsection{Search Space Refinement}\label{sec:search}
With the unified FFN and the deletion of residual-connected token mixer, we examine whether the search space from EfficientFormer is still sufficient, especially in terms of depth. 
We vary the network depth (number of blocks in each stage) and width (number of channels), and find that deeper and narrower network leads to  better accuracy ($0.2\%$ improvement), less parameters ($0.13$M reduction), and lower latency ($0.1$ms acceleration), as in Tab.~\ref{tab:rethink_design}. 
Therefore, we set this network as a new baseline (accuracy $80.5\%$) to validate subsequent design modifications, and enable a deeper supernet for architecture search in Sec.~\ref{sec:joint_search}. 

In addition, 5-stage models with further down-sized spatial resolution ($\frac{1}{64}$) have been widely employed in efficient ViT arts~\cite{levit,chen2021mobile,liu2022uninet}. 
To justify whether we should search from a 5-stage supernet, we append an extra stage to current baseline network and verify the performance gain and overhead. 
It is noteworthy that though computation overhead is not a concern given the small feature resolution, the additional stage is parameter intensive. 
As a result, we need to shrink the network dimension (depth or width) to align parameters and latency to the baseline model for fair comparison. 
%To the best result we obtain, as in Tab.~\ref{tab:analysis}, with more parameters ($0.39$M) and latency overhead ($0.2$ms), the performance of the 5-stage model surprisingly degrades to $80.31\%$, despite with savings in MACs ($0.12$G). 
As seen in Tab.~\ref{tab:rethink_design}, the best performance of the 5-stage model surprisingly drops to $80.31\%$ with more parameters ($0.39$M) and latency overhead ($0.2$ms), despite the saving in MACs ($0.12$G). 
This aligns with our intuition that the fifth stage is computation efficient but parameter intensive.
Given that 5-stage network can not introduce more potentials in our size and speed scope, we stick to 4-stage design. 
This analysis also explains why some ViTs offer an excellent Pareto curve in MACs-Accuracy, but tend to be quite redundant in size~\cite{levit,chen2021mobile}. 
As the most important takeaway, optimizing single metric is easily trapped, and the proposed joint search in Sec.~\ref{sec:joint_search} provides a feasible solution to this issue. 

% ================= V1% ================= 
% With the deletion of explicit residual-connected local mixers, the effective depth of the network decreases. 
% To validate the necessity to reform search space and regenerate optimal compact networks, we vary $N$ and $C$ to form a deeper and narrower network and observe a 0.2\% increase in accuracy with even less parameters (12.24M) and lower latency (1.3ms). 
% We set this network as a new baseline (80.54\%) to validate subsequent design modifications, and leave the architecture optimization to the final joint search step by incorporating a deeper supernet. 

% In addition, as widely employed in \cite{}, an additional stage with further down-sized resolution (1/64) may be beneficial to performance. 
% To justify whether we should search from a 5-stage supernet, we append an extra stage to current baseline network and verify the performance gain and overhead. 
% It is noteworthy that though computation overhead is not a concern given the small feature resolution, the additional stage is parameter intensive. 
% As a result, we need to shrink the network dimension (depth or width) to align parameters and latency and give a fair comparison. 
% To the best result we obtain, as in Tab.~\ref{}, with slightly more parameters (0.4M) and latency overhead (0.16ms), the performance surprisingly degraded to 80.31\%, despite there are some savings in MACs (0.13G). 
% This aligns with our intuition that the 5th stage is computation efficient but parameter intensive. 
% Given that 5-stage network can not introduce more potentials in our size \& speed scope, we stick to 4-stage design. 
% Our analysis also provides an explanation why some ViTs (e.g. LeViT \cite{}) offer an excellent Pareto curve in MACs-accuracy, but tend to be quite redundant in size. 
% As the most important takeaway, optimizing single metric is easily trapped, and the proposed joint search in Sec.~\ref{} provides a feasible solution to this issue. 


\subsection{MHSA Improvements}\label{sec:improve_mhsa}
We then study the techniques to improve the performance of attention modules without raising extra overhead in model size and latency. 
As shown in Fig.~\ref{fig:main}{(c)}, we investigate two approaches for MHSA.
First, we inject local information into the Value matrix ($V$) by adding a depth-wise $3\times3$ CONV, which is also employed by \cite{gong2022nasvit,si2022inception}. Second, we enable communications between attention heads by adding fully connected layers across head dimensions \cite{shazeer2020talking} that are shown as Talking Head in Fig.~\ref{fig:main}{(c)}. 
With these modifications, we further boost the performance to $80.8\%$ with similar parameters and latency compared to the baseline model.

\subsection{Attention on Higher Resolution}\label{sec:higher_res}
% \georgios{any better title??: Attention at early stages or Early Attention?}
Attention mechanism is beneficial to performance. However, applying it to high-resolution features harms mobile efficiency since it has quadratic time complexity corresponding to spatial resolution.
We investigate strategies to efficiently apply MHSA to higher resolution (early stages).
Recall that in the current baseline network obtained in Sec.~\ref{sec:improve_mhsa}, MHSA is only employed in the last stage with $\frac{1}{32}$ spatial resolution of the input images. 
We apply extra MHSA to the second last stage with $\frac{1}{16}$ feature size, and observe $0.9\%$ gain in accuracy. 
On the down side, the inference speed slows down by almost $2.7\times$. Thus, it is necessary to properly reduce complexity of the attention modules. 

Although some work propose window-based attention~\cite{liu2021swin,dong2022cswin}, or downsampled Keys and Values \cite{li2022next} to alleviate this problem, we find that they are not best-suited options for mobile deployment. Window-based attention is difficult to accelerate on mobile devices due to the sophisticated window partitioning and reordering. As for downsampling Keys ($K$) and Values ($V$) in \cite{li2022next}, full resolution Queries ($Q$) are required to preserve the output resolution ($\mathbf{Out}$) after attention matrix multiplication:
\begin{equation}
\small
    \mathbf{Out}_{[B, H, N, C]} = ( Q_{[B, H, N, C]} \cdot K^T_{[B, H, C, \frac{N}{2}]} ) \cdot V_{[B, H, \frac{N}{2}, C]},
\end{equation}
where $B$, $H$, $N$, $C$ denotes batch size, number of heads, number of tokens, and channel dimension respectively. 
Based on our test, the latency of the model merely drops to $2.8$ms, which is still $2\times$ slower than the baseline model.

Therefore, to perform MHSA at the earlier stages of the network, we downsample all Query, Key, and Value to a fixed spatial resolution ($\frac{1}{32}$) and interpolate the outputs from the attention back to the original resolution to feed into the next layer, as shown in Fig.~\ref{fig:main}({(d)\&(e)}).
We refer to this method as Stride Attention. 
As in Tab.~\ref{tab:rethink_design}, this simple approximation significantly reduces the latency from $3.5$ms to $1.5$ms and preserves a competitive accuracy ($81.5\%$ \emph{vs.} $81.7\%$).  

\subsection{Dual-Path Attention Downsampling}\label{sec:subsample}
Most vision backbones utilize strided convolutions or pooling layers to perform a static and local downsampling and form a hierarchical structure. 
Some recent works start to explore attention downsampling. For instance, LeViT~\cite{levit} and UniNet~\cite{liu2022uninet} propose to halve feature resolution via attention mechanism to enable context-aware downsampling with the global receptive field. Specifically, the number of tokens in Query is reduced by half so that the output from the attention module is downsampled:
\begin{equation}
\small
    \mathbf{Out}_{[B, H, \frac{N}{2}, C]} = ( Q_{[B, H, \frac{N}{2}, C]} \cdot K^T_{[B, H, C, N]} ) \cdot V_{[B, H, N, C]}.
\end{equation}
However, it is nontrivial to decide how to reduce the number of tokens in Query. 
Graham \emph{et al.} empirically use pooling to downsample Query~\cite{levit}, while Liu \emph{et al.} propose to search for local or global approaches~\cite{liu2022uninet}. 
To achieve acceptable inference speed on mobile devices, applying attention downsampling to early stages with high resolution is not favorable, restricting the values of existing works that search different downsampling approaches at higher-resolution.

Instead, we propose a combined strategy, which is dual-path attention downsampling, that wields both locality and global dependency, as in Fig.~\ref{fig:main}{(f)}. 
To get downsampled Queries, we use pooling as static local downsampling,  $3\times 3$ DWCONV as learnable local downsampling, and combine and project the results into Query dimension. In addition, the attention downsampling module is residual connected to a regular strided CONV to form a local-global manner, similar to the downsampling bottlenecks~\cite{he2016deep} or inverted bottlenecks~\cite{sandler2018mobilenetv2}.
As shown in Tab.~\ref{tab:rethink_design}, with slightly more parameters and latency overhead, we further improve the accuracy to $81.8\%$ with dual-path attention downsampling, which also has better performance than only using attention module for subsampling, \emph{i.e.}, attention downsampling. 

% \textcolor{red}{For instance, our attention downsample module (Sec.3.5) incorporates hybrid token sampling, \emph{i.e.}, static \& learnable Queries and local-global dual-path structure, and achieves $0.4\%$ higher accuracy compared to the original one [22]. }
% ================= V1% ================= 
% Most vision backbones utilize strided convolutions or pooling layers to perform a static and local downsampling and form a hierarchical structure. 
% LeViT \cite{} and UniNet \cite{} propose to halve feature resolution via attention thus enabling context-aware downsampling with global receptive field. Specifically, the number of tokens in Query are reduced to half, such that the attention output is downsampled. 
% \begin{equation}
% \small
%     \mathbf{Out}_{[B, H, \frac{N}{2}, C]} = ( Q_{[B, H, \frac{N}{2}, C]} \cdot K^T_{[B, H, C, N]} ) \cdot V_{[B, H, N, C]}
% \end{equation}
% However, it is nontrivial to decide how to reduce the tokens in Query. 
% \cite{} empirically use local pooling or global fully connected layers to downsample Query, while \cite{} propose to search for local or global approaches. 
% In our mobile deployment scope, it is not feasible to apply attention downsampling to early stages with high resolution, which restricts the value of searching different methods. 
% Instead, we propose a combined strategy that wields both locality and global dependency, as in Fig.~\ref{fig:main}. 
% To generate Queries, we use pooling as static local downsampling, depth wise $3\times 3$ convolution as learnable local downsampling, and fully connected layer as global downsampling, and combine and project the results into Query dimension. In addition, the attention downsampling module is residual connected to a regular strided convolution to improve stability, similar to the downsampling bottlenecks or inverted bottlenecks in \cite{}. 
% As in Tab.~\ref{tab:analysis}, with slight parameter and latency overhead, we further boost the accuracy to $81.8\%$ with attention downsampling. 


\section{EfficientFormerV2}
As discussed, current arts merely focus on optimizing one metric, thus are either redundant in size~\cite{efficientformer} or slow in inference~\cite{mehta2021mobilevit}. 
To find the most suitable vision backbones for mobile deployment, we propose to jointly optimize model size and speed. 
Furthermore, the network designs in Sec.~\ref{sec:3rethink} %prefer
favor a deeper network architecture (Sec.~\ref{sec:search}) and more attentions (Sec.~\ref{sec:higher_res}), calling for an improved search space and algorithm. 
%In the following, 
In what follows, we present the supernet design of EfficientFormerV2 and its search algorithm. 

\subsection{Design of EfficientFormerV2}
As discussed in Sec.~\ref{sec:search}, we employ a 4-stage hierarchical design which obtains feature sizes in  $\{\frac{1}{4},\frac{1}{8},\frac{1}{16},\frac{1}{32}\}$ of the input resolution. 
%Similar to EfficientFormer
Similar to its predecessor~\cite{efficientformer}, EfficientFormerV2 starts with a small kernel convolution \texttt{stem} to embed input image instead of using inefficient %non-overlap patch embedding, 
embedding of non-overlapping patches,
\begin{equation}
\small
    \mathbb{X}_{i|_{i=1}, j|_{j=1}}^{B,C_{j|_{j=1}},\frac{H}{4},\frac{W}{4}} = \texttt{stem}(\mathbb{X}_0^{B,3,H,W}),
\end{equation}
where $B$ denotes the batch size, $C$ refers to channel dimension (also represents the width of the network), $H$ and $W$ are the height and width of the feature, $\mathbb{X}_j$ is the feature in stage $j$, $j \in \{1,2,3,4\}$, and $i$ indicates the $i$-th layer. 
The first two stages capture local information on high resolutions; thus we only employ the unified FFN (\texttt{FFN}, Fig.~\ref{fig:main}{(b)}), 
\begin{equation}
\small
        \mathbb{X}_{i+1, j}^{B,C_j,\frac{H}{2^{j+1}},\frac{W}{2^{j+1}}} = \texttt{S}_{i,j} \cdot \texttt{FFN}^{C_j,E_{i,j}}(\mathbb{X}_{i,j}) + \mathbb{X}_{i,j},
        \label{eq:local}
\end{equation}
where $\texttt{S}_{i,j}$ is a learnable layer scale \cite{yu2021metaformer} and the $\texttt{FFN}$ is constructed by two properties: stage width $C_j$ and a per-block expansion ratio $E_{i,j}$.
%where the $\texttt{FFN}$ is constructed by two properties: stage width $C_j$ and a per-block expansion ratio $E_{i,j}$, and $\texttt{S}_{i,j}$ is a learnable layer scale\todo{~\cite{}}. 
Note that each \texttt{FFN} is residual connected. 
In the last two stages, both local \texttt{FFN} and global \texttt{MHSA} blocks are used. Therefore,  on top of Eqn.~\ref{eq:local}, global blocks are defined as:
\begin{equation}
\small
        \mathbb{X}_{i+1,j}^{B,C_j,\frac{H}{2^{j+1}},\frac{W}{2^{j+1}}} = \texttt{S}_{i,j} \cdot \texttt{MHSA}(\texttt{Proj}(\mathbb{X}_{i,j})) + \mathbb{X}_{i,j},
        \label{eq:global}
\end{equation}
where Queries ($Q$), Keys ($K$), and Values ($V$) are projected from input features through linear layers $Q, K, V \leftarrow \texttt{Proj}(\mathbb{X}_{i,j})$, and 
\begin{equation}
\small
  \texttt{MHSA}(Q,K,V) = \texttt{Softmax}(Q\cdot K^T + \texttt{ab}) \cdot V,
\end{equation}
with \texttt{ab} as a learnable attention bias for position encoding. 


\subsection{Jointly Optimizing Model Size and Speed} \label{sec:joint_search}
Though the baseline network EfficientFormer~\cite{efficientformer} is found by latency-driven search and wields fast inference speed on mobile, there are two major drawbacks for the search algorithm. 
First, the search process is merely constrained by speed, resulting in the final models being parameter redundant, as in Fig.~\ref{fig:bubble}.
Second, it only searches for depth (number of blocks $N_j$ per stage) and stage width $C_j$, which is in a \emph{coarse-grained} manner. In fact, the majority of computations and parameters of the network are in $\texttt{FFN}$s, and the parameter and computation complexity are linearly related to its expansion ratio $E_{i,j}$. $E_{i,j}$ can be specified independently for each $\texttt{FFN}$ without the necessity to be identical. Thus, searching $E_{i,j}$ enables a more \emph{fine-grained} search space where the computations and parameters can distribute \emph{flexibly} and \emph{non-uniformly} within each stage. 
This is a missing property in most recent ViT NAS arts \cite{gong2022nasvit,liu2022uninet,efficientformer}, where $E_{i,j}$ remains identical per stage. 
We propose a search algorithm that enables a flexible per-block configuration, with joint constraints on size and speed, and finds vision backbones best suited for mobile devices.  

\subsubsection{Search Objective} \label{sec:objective}
% \textcolor{red}{tend to formulate MES as our search objective, may need rephrase}
% As discussed, optimizing the Pareto curve merely on one metric easily enters a pitfall that the good performance is achieved by sacrificing too much on another.
First, we introduce the metric guiding our joint search algorithm. Given the fact that the size and latency of a network all matter when evaluating mobile-friendly models, we consider a generic and fair metric that better understands the performance of a network on mobile devices.
% The size, latency, and performance of a network all matter when evaluating mobile-friendly models. The satisfactory performance of one metric does not necessarily indicate the high performance of other metrics, \emph{e.g.,}, a classification model with high accuracy might not have a small size. Thus, we consider a generic and fair metric that can better understand the performance of a network on mobile devices.
Without loss of generality, we define a \underline{M}obile \underline{E}fficiency \underline{S}core (\texttt{MES}):
\begin{equation}
\small
    \texttt{MES} = Score \cdot \prod_i (\frac{M_i}{U_i})^{-\alpha_i},
    \label{eq:mescore}
\end{equation}
where $i \in \{ {size}, latency, ...\}$ and $\alpha_i \in (0, 1]$ indicating the corresponding importance. $M_i$, and $U_i$ represent the metric and its unit.
$Score$ is a pre-defined base score set as $100$ for simplicity.
Model size is calculated by the number of parameters, and latency is measured as running time when deploying models on devices.
Since we focus on mobile deployment, the size and speed of MobileNetV2 are used as the unit.
Specifically, we define $U_{size}=3\text{M}$, and $U_{latency}$ as $1$ms latency on iPhone 12 (iOS 16) deployed with CoreMLTools~\cite{coreml2021}. To emphasize speed,
%we set $\alpha_{latency}$ as 1.0, while $\alpha_{size}$ as 0.5.
we set $\alpha_{latency} = 1.0$ and $\alpha_{size} = 0.5$.
% Decreasing size ($U_{size}$) and inference time ($U_{latency}$) 
Decreasing size and latency
can lead to a higher \texttt{MES}, and we search for Pareto optimality on \texttt{MES}-Accuracy.
The form of \texttt{MES} is general and can be extended to other metrics of interest, such as inference-time memory footprint and energy consumption. Furthermore, the importance of each metric is easily adjustable by appropriately defining $\alpha_i$. 



% Without loss of generality, we define a \underline{M}obile \underline{E}fficiency \underline{S}core (\texttt{MES}) as follows,
% \begin{equation}
%     \texttt{MES} = P \cdot \prod_i (\frac{M_i}{U_i})^{-\alpha_i},
%     \label{eq:mescore}
% \end{equation}
% % where \texttt{S} is a predefined base score (i.e. 100), 
% where $P$ is the performance metric for a model, \emph{e.g.}, top-1 accuracy for a classification model, and $i \in \{ {size}, latency\}$ with $\alpha_i$, $M_i$, and $U_i$ indicate the corresponding weight, metric, and its unit. 
% The model size is calculated through the number of parameters and latency is measured as running time when deploying models on device.
% Since we focus on mobile deployment, the size and speed of MobileNetV2 are used as the unit.
% Specifically, we define $U_{size}$ as $3$ M parameters, and $U_{latency}$ as $0.9$ ms inference latency on iPhone 12 (iOS 16) deployed with CoreMLTools~\cite{coreml2021}. The $\alpha_i$ is set as 1.
% Increasing the model performance ($P$), decreasing the size ($U_{size}$), and accelerating the inference time ($U_{latency}$) can lead to higher \texttt{MES} score, which  also indicates a better model.
% % Intuitively, a model with 3M parameters and 1ms inference latency obtains a \texttt{meScore} of 100, while \texttt{meScore} drops to 25 on a larger model with doubled parameters (6M) and latency (2ms). 
% The form of \texttt{MES} is general and can further be extended to other metrics of interest, such as inference-time memory footprint and energy consumption, into it. Furthermore, the importance of each metric is easily adjustable by appropriately defining $\alpha_i$. 

\subsubsection{Search Space and SuperNet}
\noindent\textbf{Search space} consists of: (i) the depth of the network, measured by the number of blocks $N_j$ per stage, (ii) the width of the network, \emph{i.e.}, the channel dimension $C_j$ per stage, and (iii) expansion ratio $E_{i,j}$ of each \texttt{FFN}. 
The amount of \texttt{MHSA} can be seamlessly determined during depth search, which controls the preservation or deletion of a block in the supernet. Thus, we set every block as \texttt{MHSA} followed by \texttt{FFN} in the last two stages of the supernet and obtain subnetworks with the desired number of global \texttt{MHSA} by depth search. 

\noindent\textbf{Supernet} is constructed by using a slimmable network~\cite{slimmable} that executes at elastic depth and width to enable a pure evaluation-based search algorithm. 
Elastic depth can be naturally implemented through stochastic drop path augmentation \cite{huang2016deep}. As for width and expansion ratio, we follow Yu \emph{et al.}~\cite{yu2019universally} to construct switchable layers with shared weights but independent normalization layers, such that the corresponding layer can execute at different channel numbers from a predefined set, \emph{i.e.}, multiples of $16$ or $32$. 
Specifically, the expansion ratio $E_{i,j}$ is determined by the channels of the depth-wise $3\times3$ Conv in each \texttt{FFN}, and stage width $C_j$ is determined by aligning the output channels of the last projection ($1\times1$ Conv) of \texttt{FFN} and \texttt{MHSA} blocks. 
The switchable execution can be expressed as:
\begin{equation}
\small
    \hat{\mathbb{X}}_i = \gamma_c \cdot \frac{w^{:c} \cdot \mathbb{X}_i - \mu_c}{\sqrt{\sigma_c^2+\epsilon}} + \beta_c,
\end{equation}
where $w^{:c}$ refers to slicing the first $c$ filters of the weight matrix to obtain a subset of output, and $\gamma_c$, $\beta_c$, $\mu_c$, and $\sigma_c$ are the parameters and statistics of the normalization layer designated for width $c$. 
The supernet is pre-trained with Sandwich Rule~\cite{slimmable} by training the largest, the smallest, and randomly sampled two subnets at each iteration (we denote these subnets as max, min, rand-1, and rand-2 in Alg.~\ref{algorithm}).

\begin{algorithm}[]
\small
\caption{Evaluation-based search for size and speed}
\label{algorithm}
\begin{algorithmic}
\Require Latency lookup table $T : \{ \texttt{FFN}^{C,E}, \texttt{MHSA}^{C} \}$
\Ensure Subnet satisfying objectives: params, latency, or \texttt{MES}

\State $\rightarrow$ \textbf{Super-net Pretraining}: 
\For{epoch}
    \For{each iter}
        \For {subnet $\in$ \{min, rand-1, rand-2, max\} } 
            \State $\mathbb{Y} \gets \prod_i \{ \texttt{FFN}_i, \texttt{MHSA}_i \}(\mathbb{X}_i) $ 
            \State $\mathcal{L} \gets criterion(\mathbb{Y}, label)$, backpropagation
        \EndFor \Comment{Sandwich Rule}
        \State  Update parameters (AdamW~\cite{loshchilov2017decoupled})
    \EndFor 
\EndFor  \Comment{finish supernet training}
\State $\rightarrow$ \textbf{Joint search for size and speed: }
\State Initialize state  $S \gets \{ S_{N_{max}}, S_{C_{max}}, S_{E_{max}} \}$
\While{Objective not satisfied} 
\State Execute action $\hat{A} \gets {\arg\min}_A \frac{\Delta \texttt{Acc}}{\Delta \texttt{MES}}$
\State Update state frontier 
\EndWhile \Comment{get sub-net with target \texttt{MES}}

% \For{each layer $\bm n$}
% \If {$\bm \alpha_n^1 > \bm \alpha_n^0$}
% \State assign DCN
% \Else{}
% \State assign regular CONV
% \EndIf
% \EndFor
\State $\rightarrow$ \textbf{Train the searched architecture from scratch} 
% \State \Comment{get final model}
\end{algorithmic}   
\end{algorithm}

\input{tabs/1_comparison}


\noindent\textbf{Discussion.} The pruning of our supernet is partially inspired by the slimmable network~\cite{slimmable}. However, the differences are also significant. First, the search objective is different. We apply the introduced joint search objective for optimizing model size and efficiency (Sec.~\ref{sec:objective}).
Second, the search actions are different. Depth is pruned through the reduction of each \emph{block}, which is possible since we unify the design and only adopt two blocks: Feed Forward Network (Sec.~\ref{sec:mixer}) and attention block. The way of pruning the depth is different from the slimmable network.
Unifying all the flexible search actions under one joint objective has not been studied for transformers before. 
% We demonstrate our search method obtains
% \emph{light and fast} transformer backbones (Sec.5, Ln. 753), overcoming the pitfall where the searched architecture is over-compliant with a specific metric while sacrificing too much on others, \emph{e.g.,} model runs fast but has large size, as in Tab.2.

\subsubsection{Search Algorithm}
Now that search objective, search space, and supernet are formulated, we present the search algorithm.
Since the supernet is executable at elastic depth and switchable width, we can search the subnetworks with the best Pareto curve by analyzing the efficiency gain and accuracy drop with respect to each slimming action. 
We define the action pool as: 
\begin{equation}
\small
    A \in \{ A_{N[i,j]}, A_{C[j]}, A_{E[i,j]} \},
\end{equation}
where $A_{N[i,j]}$ denotes slimming each block, $A_{C[j]}$ refers to shrinking the width of a stage, and $A_{E[i,j]}$ denotes slimming each \texttt{FFN} to a smaller expansion. 
Initializing the state with full depth and width (largest subnet), we evaluate the accuracy outcome ($\Delta \texttt{Acc}$) of each frontier action on a validation partition of ImageNet-1K, which only takes about 4 GPU-minutes. 
Meanwhile, parameter reduction ($\Delta \texttt{Params}$) can be directly calculated from layer properties, \emph{i.e.}, kernel size, in-channels, and out-channels. 
We obtain the latency reduction ($\Delta \texttt{Latency}$) through a pre-built latency look-up table measured on iPhone 12 with CoreMLTools. 
With the metrics in hand, we can compute $\Delta \texttt{MES}$ through $\Delta \texttt{Params}$ and $\Delta \texttt{Latency}$, and choose the action with the minimum per-\texttt{MES} accuracy drop: $\hat{A} \gets {\arg\min}_A \frac{\Delta \texttt{Acc}}{\Delta \texttt{MES}}$.
% \begin{equation}
% \small
%     \hat{A} \gets {\arg\min}_A \frac{\Delta \texttt{Acc}}{\Delta \texttt{MES}}
% \end{equation}
It is noteworthy that though the action combination is enormous, we only need to evaluate the frontier one at each step, which is linear in complexity. Details can be found in Alg.~\ref{algorithm}. 







==> iccv2023AuthorKit/sections/4_exp.tex <==
\section{Experiments}

\input{tabs/2_detection}
% \input{iccv2023AuthorKit/tabs/ablate_search}

% \subsection{Setup}
\subsection{ImageNet-1K Classification}
\noindent\textbf{Implementation Details.}
We implement the model through PyTorch 1.12~\cite{paszke2019pytorch} and Timm library~\cite{rw2019timm}, and use $16$ NVIDIA A100 GPUs to train our models.
% We follow existing work~\cite{levit,efficientformer,yu2021metaformer,touvron2021training} to conduct experiments on ImageNet-1K dataset~\cite{deng2009imagenet}.
% For fair comparison with most works, 
We train the models from scratch by $300$ and $450$ epochs on ImageNet-1K~\cite{deng2009imagenet}, with AdamW~\cite{loshchilov2017decoupled} optimizer. 
Learning rate is set to $10^{-3}$ per $1,024$ batch size with cosine decay. 
We use a standard image resolution, \emph{i.e.}, $224\times224$, for both training and testing. 
Similar to DeiT~\cite{touvron2021training}, we use RegNetY-16GF~\cite{radosavovic2020designing} with $82.9\%$ top-1 accuracy as the teacher model for hard distillation.  
We use three testbeds to benchmark the latency:
\begin{itemize}[leftmargin=1em]
% \setlength
% \itemsep{-0.4em}
    \item \textbf{iPhone 12 - NPU.} We get the latency on iPhone 12 (iOS 16) by running the models on Neural Engine (NPU). The models (batch size of $1$) are compiled with CoreML~\cite{coreml2021}.
    % to be measured with built-in benchmark tools.
    \item \textbf{Pixel 6 - CPU.} We test model latency on Pixel 6 (Android) CPU. To obtain the latency for most works under comparison, we replace the activation from \emph{all} models to ReLU to get fair comparisons. The models (batch size of $1$) are compiled with XNNPACK~\cite{XNNPACK}.
    \item \textbf{Nvidia GPU.} We also provide the latency on a high-end GPU--Nvidia A100. The models (batch size of $64$) are deployed in ONNX~\cite{ONNX} and executed by TensorRT~\cite{TensorRT}. 
\end{itemize}
% \input{tabs/2_detection}
% % \input{tabs/3_segmentation}
% \subsubsection{Comparisons}
\noindent\textbf{Evaluation on Single Metric.}
We show the comparison results in Tab.~\ref{tab:comparison}, which includes \emph{the most recent and representative} works on vision transformers and CNNs. The works that \emph{do not have public models} or \emph{are not compatible with mobile devices}~\cite{cai2022efficientvit,deformableattention,liu2021swin2} are not contained in Tab.~\ref{tab:comparison}.
EfficientFormerV2 series achieve the SOTA results on a single metric, \emph{i.e.}, number of parameters or latency. 
For model size, EfficientFormerV2-S0 outperforms EdgeViT-XXS~\cite{pan2022edgevits} by $1.3\%$ top-1 accuracy with even $0.6$M fewer parameters and MobileNetV2$\times1.0$~\cite{sandler2018mobilenetv2} by $3.5\%$ top-1 with similar number of parameters. For large models, EfficientFormerV2-L model achieves identical accuracy to recent EfficientFormer-L7~\cite{efficientformer} while being $3.1\times$ smaller. 
As for speed, with comparable or lower latency, EfficientFormerV2-S2 outperforms UniNet-B1~\cite{liu2022uninet}, EdgeViT-S~\cite{pan2022edgevits}, and EfficientFormer-L1~\cite{efficientformer} by $0.8\%$, $0.6\%$ and $2.4\%$ top-1 accuracy, respectively. 
We hope the results can provide practical insight to inspire future architecture design: \emph{modern deep neural networks are robust to architecture permutation, optimizing the architecture with joint constraints, such as latency and model size, will not harm individual metrics.}



\noindent\textbf{Jointly Optimized Size and Speed.}
Further, we demonstrate the superior performance of EfficientFormerV2 when considering both model size and speed. 
Here we use \texttt{MES} as a more practical metric to assess mobile efficiency than using size or latency alone.
EfficientFormerV2-S1 outperforms MobileViT-XS~\cite{mehta2021mobilevit}, EdgeViT-XXS~\cite{pan2022edgevits}, and EdgeViT-XS~\cite{pan2022edgevits} by $4.2\%$, $4.6\%$, and $1.5\%$ top-1, respectively, with %times
far higher \texttt{MES}. With $1.8\times$ higher \texttt{MES},  EfficientFormerV2-L outperforms MobileFormer-508M~\cite{chen2021mobile} by $4.0\%$ top-1 accuracy. 
The evaluation results answer the central question raised at the beginning: \emph{with the proposed mobile efficiency benchmark (Sec.~\ref{sec:objective}), we can avoid entering a pitfall achieving seemingly good performance on one metric while sacrificing too much for others. Instead, we can obtain efficient mobile ViT backbones that are both light and fast. }


\subsection{Downstream Tasks}

\input{iccv2023AuthorKit/tabs/ablate_search}


% \todo{Recent work shows that freezing the statistics of normalization layers yields better performance in downstream tasks~\cite{li2022next}, as the training recipe in detection and segmentation usually employs a small batch size, making the calculation of running statistics less accurate. 
% We follow Li \emph{et al.}~\cite{li2022next} to apply a larger weight decay as $0.05$ and freeze the normalization layers, and demonstrate the improved results in detection and segmentation tasks, as in Tab.~\ref{tab:coco_improved} and Tab.~\ref{tab:ade20k_improved}. }

 
\noindent\textbf{Object Detection and Instance Segmentation.}  We apply EfficientFormerV2 as backbone in Mask-RCNN~\cite{he2017mask} pipeline and experiment on MS COCO 2017~\cite{lin2014microsoft}. The model is initialized with ImageNet-1K pretrained weights. We use AdamW~\cite{loshchilov2017decoupled} optimizer with an initial learning rate as $2\times10^{-4}$ and conduct training for $12$ epochs with resolution as $1333\times 800$. Following Li \emph{et al.}~\cite{li2022next}, we apply a weight decay as $0.05$ and freeze the normalization layers in the backbone.
As in Tab.~\ref{tab:coco}, with similar model size, our EfficientFormerV2-S2 outperform PoolFormer-S12~\cite{yu2021metaformer} by $6.1$ AP$^{box}$ and $4.9$ AP$^{mask}$. EfficientFormerV2-L outperforms EfficientFormer-L3~\cite{efficientformer} by $3.3$ AP$^{box}$ and $2.3$ AP$^{mask}$. 

\noindent\textbf{Semantic Segmentation.}  We perform experiments on ADE20K \cite{zhou2017scene}, a challenging scene segmentation dataset with $150$ categories. 
Our model is integrated as a feature encoder in Semantic FPN~\cite{kirillov2019panoptic} pipeline, with ImageNet-1K pretrained weights. 
We train our model on ADE20K for $40$K iterations with batch size as $32$ and learning rate as $2\times 10^{-4}$ with a poly decay by the power of $0.9$. 
We apply weight decay as $10^{-4}$ and freeze the normalization layers.
Training resolution is $512\times 512$, and we employ a single scale testing on the validation set. 
As in Tab.~\ref{tab:coco}, EfficientFormerV2-S2 outperforms PoolFormer-S12 \cite{yu2021metaformer} and EfficientFormer-L1 \cite{efficientformer} by $5.2$ and $3.5$ mIoU, respectively. 


% \input{tabs/3_segmentation}
% \input{tabs/4_ablation}

\subsection{Ablation Analysis on Search Algorithm}

We compare the proposed search algorithm with the random search and the one from EfficientFormer~\cite{efficientformer}. As seen in Tab.~\ref{tab:ablate_search}, our search algorithm obtains models with much better performance than random search, \emph{i.e.}, Random 1 and Random 2. Compared with EfficientFormer~\cite{efficientformer}, we achieve higher accuracy under similar parameters and latency, demonstrating the effectiveness of fine-grained search and joint optimization of latency and size. 
% We provide more ablations of our search algorithm in \emph{supplementary materials}.

% In addition to the analysis for design choices in Sec.~\ref{sec:3rethink}, we further study the effectiveness of the proposed search algorithm. 
% We deactivate the per-\texttt{FFN} search for $E_{i,j}$, and use latency as constraint as in \cite{efficientformer}. As in Tab.~\ref{tab:ablate_search}, our fine-grained joint search generate better subnetworks. 





==> iccv2023AuthorKit/sections/5_conclusion.tex <==
\section{Discussion and Conclusion}
In this work, we comprehensively study transformer backbones, identify inefficient designs, and introduce mobile-friendly novel architectural changes.
We further propose a fine-grained joint search on size and speed and obtain the EfficientFormerV2 model family. We extensively benchmark and compare our work with existing studies on different hardware and demonstrate that EfficientFormerV2 is both lightweight, ultra-fast in inference speed and high performance. 
Since we focus on size and speed,
one future direction is to apply the joint optimization methodology to subsequent research exploring other critical metrics, such as memory footprint and CO$_2$ emission.
% EfficientFormerV2 is generated by empirically setting the size and speed as equally important to get the \texttt{MES}. %score. 
% In industry scenarios, the preference may vary. 
% In addition, 

\section{Acknowledgements}
This work is partly supported by the Army Research Office/Army Research Laboratory via grant W911-NF-20-1-0167 to Northeastern University, \and CNS1909172.

==> iccv2023AuthorKit/tabs/0_analysis.tex <==
\begin{table*}[]
\small
\centering
\caption{\textbf{Number of parameters, latency, and performance} for various design choices. The latency is tested on iPhone 12. Top-1 accuracy is obtained by validating models on ImageNet-1K for the classification task.}\label{tab:rethink_design}
\resizebox{1.0\linewidth}{!}{
\small
\begin{tabular}{cccccc}
\toprule
Section                & Method                         & \#Params (M) & MACs (G) & Latency (ms) & Top-1 (\%) \\
\hline
(Baseline)             & EfficientFormer-L1             & 12.25        & 1.30     & 1.4          & 79.2     \\
\hline
\multirow{2}{*}{Sec.~\ref{sec:mixer}} &  Pool Mixer $\rightarrow$ DWCONV$_{3\times3}$                    & 12.27        & 1.30     & 1.4          & 79.8     \\
                      & $\checkmark$ Feed Forward Network %Unified Block
                      & 12.37        & 1.33     & 1.4          & 80.3     \\
                      \hline
\multirow{2}{*}{Sec.~\ref{sec:search}} & $\checkmark$ Vary Depth and Width               & 12.24        & 1.20     & 1.3          & 80.5     \\
                      & 5-Stage Network                        & 12.63        & 1.08     & 1.5          & 80.3     \\
                      \hline
Sec.~\ref{sec:improve_mhsa}                  & $\checkmark$ Locality in $V$ \& Talking Head  & 12.25        & 1.21     & 1.3          & 80.8     \\
\hline
\multirow{2}{*}{Sec.~\ref{sec:higher_res}} & Attention at Higher Resolution & 13.10        & 1.48     & 3.5          & 81.7     \\
                      & $\checkmark$ Stride Attention              & 13.10        & 1.31     & 1.5          & 81.5     \\
                      \hline
\multirow{2}{*}{Sec.~\ref{sec:subsample}}                 &  Attention Downsampling        & 13.18        & 1.33     & 1.6          & 81.4     \\
 & $\checkmark$ Dual-Path Attention Downsampling        & 13.40        & 1.35     & 1.6          & 81.8     \\
\bottomrule
\end{tabular}
}
\end{table*}

% \begin{figure*}

% % \begin{minipage}[h]{\linewidth}
% \begin{minipage}{0.65\linewidth}
%     \centering
%     \captionof{table}{Rethink design choices.}\label{tab:rethink_design}
%     \small
% \scalebox{0.75}{
% \begin{tabular}{cccccc}
% \toprule
% Section                & Method                         & \#Params (M) & MACs (G) & Latency (ms) & Acc (\%) \\
% \hline
% (Baseline)             & a. EfficientFormer-L1             & 12.25        & 1.30     & 1.4          & 79.2     \\
% \hline
% \multirow{2}{*}{Sec.~\ref{sec:mixer}} &  Pool Mixer $\rightarrow$ DWCONV$_{3\times3}$                    & 12.27        & 1.30     & 1.4          & 79.8     \\
%                       & $\checkmark$ b. Feed Forward Network %Unified Block
%                       & 12.37        & 1.33     & 1.4          & 80.3     \\
%                       \hline
% \multirow{2}{*}{Sec.~\ref{sec:search}} & $\checkmark$ c. Vary Depth and Width               & 12.24        & 1.20     & 1.3          & 80.5     \\
%                       & 5-Stage Network                        & 12.63        & 1.08     & 1.5          & 80.3     \\
%                       \hline
% Sec.~\ref{sec:improve_mhsa}                  & $\checkmark$ d. Locality in $V$ \& Talking Head  & 12.25        & 1.21     & 1.3          & 80.8     \\
% \hline
% \multirow{2}{*}{Sec.~\ref{sec:higher_res}} & e. Attention at Higher Resolution & 13.10        & 1.48     & 3.5          & 81.7     \\
%                       & $\checkmark$ f. Stride Attention              & 13.10        & 1.31     & 1.5          & 81.5     \\
%                       \hline
% Sec.~\ref{sec:subsample}                 & $\checkmark$ g. Attention Downsampling        & 13.40        & 1.35     & 1.6          & 81.8     \\
% \bottomrule
% \end{tabular}
% }
%     \end{minipage}\hfill
%   \begin{minipage}{0.35\linewidth}
%     \centering
%     \scalebox{0.9}{
%     \includegraphics[width=\linewidth]{figures/rethink.pdf}
%     }
%     \setlength{\tabcolsep}{0.9\linewidth}
% % \begin{tabular}{C{0.2\linewidth}C{0.2\linewidth}C{0.2\linewidth}C{0.2\linewidth}C{0.2\linewidth}}
% % \small$t=2$&\small$t=6$&\small$t=10$&\small$t=14$&\small$t=16$
% % \end{tabular}
%     \captionof{figure}{Rethink design choices.}\label{fig:rethink}
%   \end{minipage}
% % \end{minipage}
% \end{figure*}

==> iccv2023AuthorKit/tabs/1_comparison.tex <==
\begin{table*}[ht]
\caption{{\textbf{Classification results on ImgeNet-1K.} 
We report the number of parameters, \emph{i.e.}, Params (M), GMACs, Training Epochs, and Top-1 accuracy for various methods.
The latency results are obtained by running models on iPhone 12 (Neural Engine) compiled with CoreMLTools, Pixel 6 (CPU) compiled with XNNPACK, and Nvidia A100 (GPU) compiled with TensorRT. The batch size is $1$ for models tested on iPhone 12 and Pixel 6, and $64$ for A100. (-) denotes unrevealed or unsupported models. $\dagger$ denotes we re-train the previous models with the exact same training recipe as our work. 
Different training seeds result in about 0.1\% fluctuation in accuracy. 
The latency is benchmarked with warmup and averaged over multiple runs, where the error ranges within 0.1 ms. 
}}
\label{tab:comparison}
\centering
\small
\scalebox{1.0}{
\begin{tabular}{lccccccccc}
\toprule
\multirow{2}{*}{Model}           & \multirow{2}{*}{Type}      & \multirow{2}{*}{Params (M)} & \multirow{2}{*}{GMACs} &  \multicolumn{3}{c}{Latency (ms)} & \multirow{2}{*}{$\texttt{MES} \uparrow$} & \multirow{2}{*}{Epochs} & \multirow{2}{*}{Top-1(\%)}  \\ \cline{5-7}
    &      &     &    &   iPhone 12  & Pixel 6  & A100     &   & &  \\
\hline
\hline
MobileNetV2$\times 1.0$     & CONV      &  3.5    & 0.3    & 0.9    & 25.3 &  5.0  & 102.9  &300& 71.8    \\
MobileNetV2$\times 1.0$ $\dagger$     & CONV      &  3.5    & 0.3    & 0.9    & 25.3 &  5.0  & 102.9  &300& 72.2    \\
MobileViT-XS       & Hybrid    &    2.3   & 0.7    & 7.3  & 64.4  & 11.7 & 15.6 &300& 74.8   \\
EdgeViT-XXS       & Hybrid    &   4.1    &  0.6   &   2.4    & 30.9 &  11.3 & 35.6 & 300  &  74.4   \\
Hydra Attention  &   Hybrid   & 3.5      &  0.38    & 4.1      & - &  9.7 & 22.6   & 300 & 75.6  \\
\rowcolor[gray]{0.92}
EfficientFormerV2-S0  &   Hybrid   & 3.5      &  0.40    & 0.9      & 20.8 & 6.6   & 102.9 & 300 / 450 & 75.7 / 76.2   \\
\hline
MobileNetV2$\times 1.4$     & CONV      &  6.1    & 0.6    & {1.2}     & 42.8 &  7.3 &  58.4  &300& 74.7    \\
MobileNetV2$\times 1.4$ $\dagger$     & CONV      &  6.1    & 0.6    & {1.2}     & 42.8 &  7.3 &  58.4  &300& 76.7    \\
MobileNetV3-L    & CONV      &  5.4    & 0.22   & 15.8    & - &  7.2 &  4.7  & 300 & 75.2    \\
FBNet-V3     & CONV      &  5.6    & 0.39   & 1.0    & - &  7.9 &  73.2  & 300 & 75.1    \\
EfficientNet-B0 & CONV      &  5.3  &  0.4   & 1.4            & 29.4 & 10.0  & 53.7  & 350 &   77.1  \\
DeiT-T          & Attention & 5.9       & 1.2      &    9.2  & 66.6 & 7.1    & 7.8 &300& 74.5    \\
EdgeViT-XS       & Hybrid    &   6.7    &  1.1   & 3.6  & 55.5 & 14.3 & 18.6 & 300 &   77.5  \\
LeViT-128S       & Hybrid    & 7.8      & 0.31     & 19.9    & 15.5 & 3.4 &  3.1  & 1000 & 76.6    \\
\rowcolor[gray]{0.92}
EfficientFormerV2-S1  &   Hybrid   & 6.1      &  0.65    & 1.1     & 33.3  &   8.8  &  63.8 & 300 / 450 & 79.0 / 79.7   \\
\hline
EfficientNet-B3 & CONV      & 12.0        & 1.8     &  5.3        & 123.8 & 35.0    & 9.4  & 350  & 81.6   \\
PoolFormer-s12  & Pool      &    12     & 2.0     &  1.5  & 82.4 & 14.5  & 33.3  & 300 & 77.2     \\
LeViT-192       & Hybrid    & 10.9      & 0.66     & 29.6 &30.1  &  5.2 &  1.8  & 1000 & 80.0    \\
MobileFormer-508M       & Hybrid    &    14.0   & 0.51    &  6.6  & 55.2 & 14.6  & 7.0 & 450 & 79.3    \\
UniNet-B1       & Hybrid    &    11.5   & 1.1    &  2.2     & 57.7  &  16.9& 23.2 & 300 & 80.8    \\
EdgeViT-S       & Hybrid    &   11.1    &   1.9  &   4.6   & 92.5 &  21.2 & 11.3 & 300 &  81.0   \\
EfficientFormer-L1       & Hybrid    &    12.3   & 1.3    & 1.4  & 50.7 & 8.4 & 35.3 & 300 & 79.2    \\
\rowcolor[gray]{0.92}
EfficientFormerV2-S2  &   Hybrid   &  12.6  &  1.25    & 1.6     & 57.2 &  14.5  & 30.5 & 300 / 450 & 81.6 / 82.0     \\
\hline
ResNet50        & CONV      &    25.5     & 4.1     & 2.5      &  167.5 & 9.0   & 13.7  &300& 78.5    \\
ResNet50 $\dagger$        & CONV      &    25.5     & 4.1     & 2.5      &  167.5 & 9.0   & 13.7  &300& 80.5    \\
ConvNext-T & CONV      &   29.0   &  4.5  &   83.7       & 340.5 &   28.8  & 0.4 & 300 & 82.1 \\
ResMLP-S24       & SMLP      &  30     & 6.0     & 7.6   & 325.4 & 17.4   &  4.2 &300& 79.4    \\
PoolFormer-s24  & Pool      &    21     & 3.6      &  2.4  & 154.3 & 28.2    & 15.7 & 300 & 80.3   \\
PoolFormer-s36  & Pool      &    31     & 5.2      &  3.5   & 224.9 & 41.2   &  8.9  & 300 & 81.4   \\
DeiT-S          & Attention & 22.5      & 4.5    &      11.8 & 218.2 & 15.5   &  3.1 &300& 81.2     \\
PVT-Small       & Attention &    24.5      & 3.8    &    24.4  & - & 23.8    &  1.4  &300& 79.8    \\
T2T-ViT-14      & Attention & 21.5      & 4.8     & -        & - & 21.0     & - &310& 81.5     \\
Swin-Tiny       & Attention &    29      & 4.5     & -       & - &22.0 & -  &300& 81.3    \\
CSwin-T       & Attention &    23      & 4.3       & -       & - & 28.7    & -  &300& 82.7  \\
LeViT-256       & Hybrid    & 18.9      & 1.12     & 31.4 & 50.7 & 6.7  &  1.3  & 1000 & 81.6    \\
LeViT-384       & Hybrid    & 39.1      & 2.35     & 48.8 & 102.2 & 10.2  &  0.6  & 1000 & 82.6    \\
Convmixer-768   & Hybrid    &  21.1 & 20.7  & 11.6  &  - & -  & 3.3 & 300 &    80.2   \\
NasViT-Supernet   & Hybrid    &  - &  1.9  &  -  &   - &  -  &  - &  360 &    82.9  \\
EfficientFormer-L3       & Hybrid    &    31.3   & 3.9    &   2.7  & 151.9 & 13.9  & 11.5 & 300 & 82.4    \\
EfficientFormer-L7      & Hybrid    &    82.1   & 10.2    &  6.6  & 392.9 & 30.7  & 2.9 & 300 & 83.3    \\
\rowcolor[gray]{0.92}
EfficientFormerV2-L  &   Hybrid   & 26.1  & 2.56 & 2.7     & 117.7 &   22.5 & 12.6  & 300 / 450 & 83.3 / 83.5    \\
\hline
\rowcolor[gray]{0.92}
Supernet  &   Hybrid   & 37.1  & 3.57 & 4.2     & - &   -  & 6.8  & 300 & 83.5    \\
\bottomrule
\end{tabular}
}
\end{table*}



==> iccv2023AuthorKit/tabs/2_detection.tex <==
% \begin{table*}[h]
% \centering
% \small
% \caption{
% \textbf{Object detection \&
% instance segmentation} on MS COCO 2017 with the Mask RCNN pipeline.
% \textbf{Semantic segmentation} on ADE20K by using models as the feature encoder in Semantic FPN.
% }
% % \resizebox{1\linewidth}{!}{
% % \begin{tabular}{c|c|cccccc}
% % \toprule
% % \multirow{2}{*}{Backbone} & \multirow{2}{*}{Params (M)} & \multicolumn{6}{c}{Detection \& Instance Segmentation}  \\ \cline{3-8}
% %                           &                         & AP$^{box}$    & AP$^{box}_{50}$   & AP$^{box}_{75}$   & AP$^{mask}$    & AP$^{mask}_{50}$   & AP$^{mask}_{75}$      \\
% %                           \hline
% %                           \hline
% % ResNet18                  &     11.7        & 34.0   & 54.0    & 36.7    & 31.2   & 51.0    & 32.7       \\
% % PoolFormer-S12            &     12.0          & 37.3   & 59.0    & 40.1    & 34.6   & 55.8    & 36.9        \\
% % EfficientFormer-L1        &     12.3              & 37.9   & 60.3    & 41.0    & 35.4   & 57.3    & 37.3       \\
% % \rowcolor[gray]{0.92}
% % EfficientFormerV2-S2      &     12.6              &  38.9  &  60.3   & 42.4  &    35.5    &   57.2      &  37.8      \\
% % \hline
% % ResNet50                  &      25.5           & 38.0   & 58.6    & 41.4    & 34.4   & 55.1    & 36.7      \\
% % PoolFormer-S24            &     21.0            & 40.1   & 62.2    & 43.4    & 37.0   & 59.1    & 39.6     \\
% % Swin-T                    &     29.0              & 42.2   & 64.4    & 46.2    & 39.1   & 64.6    & 42.0      \\
% % % PVTv2-B2                  &                         & 45.3   & 67.1    & 49.6    & 41.2   & 64.2    & 44.4    \\
% % % Twins-SVT-S               &                         & 43.4   & 66.0    & 47.3    & 40.3   & 63.2    & 43.4      \\
% % EfficientFormer-L3        &         31.3     & 41.4   & 63.9    & 44.7    & 38.1   & 61.0    & 40.4      \\
% % % CSwin-T                   &                         & 46.7   & 68.6    & 51.3    & 42.2   & 65.6    & 45.4     \\
% % \rowcolor[gray]{0.92}
% % EfficientFormerV2-L       &       26.1      & 42.4   &  64.2  &  46.7   &  38.7   &  61.1   & 41.6           \\
% % \bottomrule
% % \end{tabular}
% \begin{tabular}{c|c|cccccc|c}
% \toprule
% \multirow{2}{*}{Backbone} & \multirow{2}{*}{Params (M)} & \multicolumn{6}{c}{Detection \& Instance Segmentation} & \multicolumn{1}{c}{Semantic}  \\ \cline{3-9}
%                           &                         & AP$^{box}$    & AP$^{box}_{50}$   & AP$^{box}_{75}$   & AP$^{mask}$    & AP$^{mask}_{50}$   & AP$^{mask}_{75}$   & mIoU   \\
%                           \hline
%                           \hline
% ResNet18                  &     11.7        & 34.0   & 54.0    & 36.7    & 31.2   & 51.0    & 32.7   & 32.9   \\
% PoolFormer-S12            &     12.0          & 37.3   & 59.0    & 40.1    & 34.6   & 55.8    & 36.9     & 37.2  \\
% EfficientFormer-L1        &     12.3              & 37.9   & 60.3    & 41.0    & 35.4   & 57.3    & 37.3   &  38.9  \\
% % EfficientFormerV2-S2      &     12.6              &  38.9  &  60.3   & 42.4  &    35.5    &   57.2      &  37.8   &   \\
% \rowcolor[gray]{0.92}
% EfficientFormerV2-S2     &     12.6              &  43.4  &  65.4   & 47.5  &    39.5    &   62.4      &  42.2   & 42.4  \\
% \hline
% ResNet50                  &      25.5           & 38.0   & 58.6    & 41.4    & 34.4   & 55.1    & 36.7  &  36.7  \\
% PoolFormer-S24            &     21.0            & 40.1   & 62.2    & 43.4    & 37.0   & 59.1    & 39.6  &  40.3 \\
% Swin-T                    &     29.0              & 42.2   & 64.4    & 46.2    & 39.1   & 64.6    & 42.0   & 41.5  \\
% % PVTv2-B2                  &                         & 45.3   & 67.1    & 49.6    & 41.2   & 64.2    & 44.4    \\
% % Twins-SVT-S               &                         & 43.4   & 66.0    & 47.3    & 40.3   & 63.2    & 43.4      \\
% EfficientFormer-L3        &         31.3     & 41.4   & 63.9    & 44.7    & 38.1   & 61.0    & 40.4   &  43.5 \\
% % CSwin-T                   &                         & 46.7   & 68.6    & 51.3    & 42.2   & 65.6    & 45.4     \\
% % EfficientFormerV2-L       &       26.1      & 42.4   &  64.2  &  46.7   &  38.7   &  61.1   & 41.6    &       \\
% \rowcolor[gray]{0.92}
% EfficientFormerV2-L      &       26.1      & 44.7   &  66.3  &  48.8   &  40.4   &  63.5   & 43.2     &   45.2   \\
% \bottomrule
% \end{tabular}
% % }
% \label{tab:coco}
% \end{table*}


% old ##############

% \begin{table*}[]
% \small
%     % \caption{Global caption}
%     \begin{minipage}{.6\linewidth}
%       \caption{
% \textbf{Object detection \&
% instance segmentation} on MS COCO 2017 with the Mask RCNN pipeline.}
%       % \centering
%       \resizebox{1\linewidth}{!}{
%         \begin{tabular}{l|c|cccccc|c}
% \toprule
% \multirow{2}{*}{Backbone} & \multirow{2}{*}{Params (M)} & \multicolumn{6}{c}{Detection \& Instance Segmentation} & \multicolumn{1}{c}{Semantic}  \\ \cline{3-9}
%                           &                         & AP$^{box}$    & AP$^{box}_{50}$   & AP$^{box}_{75}$   & AP$^{mask}$    & AP$^{mask}_{50}$   & AP$^{mask}_{75}$   & mIoU   \\
%                           \hline
%                           \hline
% ResNet18                  &     11.7        & 34.0   & 54.0    & 36.7    & 31.2   & 51.0    & 32.7   & 32.9   \\
% PoolFormer-S12            &     12.0          & 37.3   & 59.0    & 40.1    & 34.6   & 55.8    & 36.9     & 37.2  \\
% EfficientFormer-L1        &     12.3              & 37.9   & 60.3    & 41.0    & 35.4   & 57.3    & 37.3   &  38.9  \\
% % EfficientFormerV2-S2      &     12.6              &  38.9  &  60.3   & 42.4  &    35.5    &   57.2      &  37.8   &   \\
% \rowcolor[gray]{0.92}
% EfficientFormerV2-S2     &     12.6              &  43.4  &  65.4   & 47.5  &    39.5    &   62.4      &  42.2   & 42.4  \\
% \hline
% ResNet50                  &      25.5           & 38.0   & 58.6    & 41.4    & 34.4   & 55.1    & 36.7  &  36.7  \\
% PoolFormer-S24            &     21.0            & 40.1   & 62.2    & 43.4    & 37.0   & 59.1    & 39.6  &  40.3 \\
% Swin-T                    &     29.0              & 42.2   & 64.4    & 46.2    & 39.1   & 64.6    & 42.0   & 41.5  \\
% % PVTv2-B2                  &                         & 45.3   & 67.1    & 49.6    & 41.2   & 64.2    & 44.4    \\
% % Twins-SVT-S               &                         & 43.4   & 66.0    & 47.3    & 40.3   & 63.2    & 43.4      \\
% EfficientFormer-L3        &         31.3     & 41.4   & 63.9    & 44.7    & 38.1   & 61.0    & 40.4   &  43.5 \\
% % CSwin-T                   &                         & 46.7   & 68.6    & 51.3    & 42.2   & 65.6    & 45.4     \\
% % EfficientFormerV2-L       &       26.1      & 42.4   &  64.2  &  46.7   &  38.7   &  61.1   & 41.6    &       \\
% \rowcolor[gray]{0.92}
% EfficientFormerV2-L      &       26.1      & 44.7   &  66.3  &  48.8   &  40.4   &  63.5   & 43.2     &   45.2   \\
% \bottomrule
% \end{tabular}}\label{tab:coco}
%     \end{minipage}% 
%     \hfill
%     \begin{minipage}{.38\linewidth}
%       % \centering
%         \caption{
% % Ablation on the proposed fine-grained search with joint constraints on size and speed, from the same supernet in Tab.~\ref{tab:comparison}
% \textbf{Ablation analysis of search algorithms.} Our proposed fine-grained search with joint constraints on size and speed achieves better results than random search and the coarse-grained, single objective search from EfficientFormer~\cite{efficientformer}. 
% Latency is measured on iPhone 12.
% }
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{l|c|c|c}
% \toprule
% % \multicolumn{3}{c|}{Search in \cite{efficientformer}} & \multicolumn{3}{c}{Ours} \\
% % \hline
% % Params   & Latency   & Top-1  & Params & Latency & Top-1 \\
% % (M)      & (ms)      & (\%)   & (M)    & (ms)    & (\%)  \\
% % \hline
% % 6.9      & 1.15      & 79.1   & 7.0    & 1.15    & 79.4  \\
% % 3.1      & 0.90      & 74.2   & 3.1    & 0.90    & 75.0  \\
% Search Algorithm & Params (M)& Latency (ms) & Top-1 ($\%$) \\ \hline
% Random 1    &    3.5    &   1.0   &   74.7 \\
% Random 2    &    3.5    &   1.0   &    75.0  \\
% \rowcolor[gray]{0.92}
% EfficientFormerV2 (Ours) &    3.5    &   0.9      &   75.7   \\
% \hline
% EfficientFormer~\cite{efficientformer} & 3.1 & 0.9 & 74.2 \\
% \rowcolor[gray]{0.92}
% EfficientFormerV2 (Ours) &3.1 & 0.9 & 75.0 \\ 
% % EfficientFormer~\cite{efficientformer} & 6.9 & 1.2 & 79.1 \\ 
% % \rowcolor[gray]{0.92}
% % EfficientFormerV2 (Ours) &7.0 & 1.2 & 79.4 \\ 
% \bottomrule
% \end{tabular}}\label{tab:ablate_search}
%     \end{minipage} 

% \end{table*}

\begin{table*}[]
    \centering
      \caption{
\textbf{Object detection \&
instance segmentation} on MS COCO 2017 with the Mask RCNN pipeline.}
      % \centering
      \small
      \resizebox{1\linewidth}{!}{
        \begin{tabular}{l|c|cccccc|c}
\toprule
\multirow{2}{*}{Backbone} & \multirow{2}{*}{Params (M)} & \multicolumn{6}{c}{Detection \& Instance Segmentation} & \multicolumn{1}{c}{Semantic}  \\ \cline{3-9}
                          &                         & AP$^{box}$    & AP$^{box}_{50}$   & AP$^{box}_{75}$   & AP$^{mask}$    & AP$^{mask}_{50}$   & AP$^{mask}_{75}$   & mIoU   \\
                          \hline
                          \hline
ResNet18                  &     11.7        & 34.0   & 54.0    & 36.7    & 31.2   & 51.0    & 32.7   & 32.9   \\
PoolFormer-S12            &     12.0          & 37.3   & 59.0    & 40.1    & 34.6   & 55.8    & 36.9     & 37.2  \\
EfficientFormer-L1        &     12.3              & 37.9   & 60.3    & 41.0    & 35.4   & 57.3    & 37.3   &  38.9  \\
% EfficientFormerV2-S2      &     12.6              &  38.9  &  60.3   & 42.4  &    35.5    &   57.2      &  37.8   &   \\
\rowcolor[gray]{0.92}
EfficientFormerV2-S2     &     12.6              &  43.4  &  65.4   & 47.5  &    39.5    &   62.4      &  42.2   & 42.4  \\
\hline
ResNet50                  &      25.5           & 38.0   & 58.6    & 41.4    & 34.4   & 55.1    & 36.7  &  36.7  \\
PoolFormer-S24            &     21.0            & 40.1   & 62.2    & 43.4    & 37.0   & 59.1    & 39.6  &  40.3 \\
Swin-T                    &     29.0              & 42.2   & 64.4    & 46.2    & 39.1   & 64.6    & 42.0   & 41.5  \\
% PVTv2-B2                  &                         & 45.3   & 67.1    & 49.6    & 41.2   & 64.2    & 44.4    \\
% Twins-SVT-S               &                         & 43.4   & 66.0    & 47.3    & 40.3   & 63.2    & 43.4      \\
EfficientFormer-L3        &         31.3     & 41.4   & 63.9    & 44.7    & 38.1   & 61.0    & 40.4   &  43.5 \\
% CSwin-T                   &                         & 46.7   & 68.6    & 51.3    & 42.2   & 65.6    & 45.4     \\
% EfficientFormerV2-L       &       26.1      & 42.4   &  64.2  &  46.7   &  38.7   &  61.1   & 41.6    &       \\
\rowcolor[gray]{0.92}
EfficientFormerV2-L      &       26.1      & 44.7   &  66.3  &  48.8   &  40.4   &  63.5   & 43.2     &   45.2   \\
\bottomrule
\end{tabular}}\label{tab:coco}
\end{table*}



==> iccv2023AuthorKit/tabs/3_segmentation.tex <==
\begin{table}[]
\centering
\small
\caption{\textbf{Semantic segmentation} on ADE20K. EfficientFormerV2 models are integrated as feature encoder in Semantic FPN.}
\begin{tabular}{c|c|c}
\toprule
Backbone             & Params (M) & mIoU \\
\hline
ResNet18             & 11.7 & 32.9 \\
PoolFormer-S12       & 12.0 & 37.2 \\
EfficientFormer-L1   & 12.3 & 38.9 \\
\rowcolor[gray]{0.92}
EfficientFormerV2-S2 & 12.6 & 39.5 \\
\bottomrule
\end{tabular}
\label{tab:ade20k}
\end{table}

==> iccv2023AuthorKit/tabs/4_ablation.tex <==
\begin{table}[]
\centering
\small
\caption{
% Ablation on the proposed fine-grained search with joint constraints on size and speed, from the same supernet in Tab.~\ref{tab:comparison}
\textbf{Ablation of search algorithms.} We achieve better results than random search and the coarse-grained, single objective search from EfficientFormer~\cite{efficientformer}. 
Latency is measured on iPhone 12.
}
% \begin{tabular}{ccc|ccc}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
% \multicolumn{3}{c|}{Search in \cite{efficientformer}} & \multicolumn{3}{c}{Ours} \\
% \hline
% Params   & Latency   & Top-1  & Params & Latency & Top-1 \\
% (M)      & (ms)      & (\%)   & (M)    & (ms)    & (\%)  \\
% \hline
% 6.9      & 1.15      & 79.1   & 7.0    & 1.15    & 79.4  \\
% 3.1      & 0.90      & 74.2   & 3.1    & 0.90    & 75.0  \\
Search Algorithm & Params (M)& Latency (ms) & Top-1 ($\%$) \\ \hline
Random 1    &    3.5    &   1.0   &   74.7 \\
Random 2    &    3.5    &   1.0   &    75.0  \\
\rowcolor[gray]{0.92}
EfficientFormerV2 (Ours) &    3.5    &   0.9      &   75.7   \\
\hline
EfficientFormer~\cite{efficientformer} & 3.1 & 0.9 & 74.2 \\
\rowcolor[gray]{0.92}
EfficientFormerV2 (Ours) &3.1 & 0.9 & 75.0 \\ 
% EfficientFormer~\cite{efficientformer} & 6.9 & 1.2 & 79.1 \\ 
% \rowcolor[gray]{0.92}
% EfficientFormerV2 (Ours) &7.0 & 1.2 & 79.4 \\ 
\bottomrule
\end{tabular}}
\label{tab:ablate_search}
\end{table}

==> iccv2023AuthorKit/tabs/ablate_search.tex <==
\begin{table}[]
\small
    \centering
        \caption{
% Ablation on the proposed fine-grained search with joint constraints on size and speed, from the same supernet in Tab.~\ref{tab:comparison}
\textbf{Ablation analysis of search algorithms.} Our proposed fine-grained search with joint constraints on size and speed achieves better results than random search and the coarse-grained, single objective search from EfficientFormer~\cite{efficientformer}. 
Latency is measured on iPhone 12.
}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\toprule
% \multicolumn{3}{c|}{Search in \cite{efficientformer}} & \multicolumn{3}{c}{Ours} \\
% \hline
% Params   & Latency   & Top-1  & Params & Latency & Top-1 \\
% (M)      & (ms)      & (\%)   & (M)    & (ms)    & (\%)  \\
% \hline
% 6.9      & 1.15      & 79.1   & 7.0    & 1.15    & 79.4  \\
% 3.1      & 0.90      & 74.2   & 3.1    & 0.90    & 75.0  \\
Search Algorithm & Params (M)& Latency (ms) & Top-1 ($\%$) \\ \hline
Random 1    &    3.5    &   1.0   &   74.7 \\
Random 2    &    3.5    &   1.0   &    75.0  \\
\rowcolor[gray]{0.92}
EfficientFormerV2 (Ours) &    3.5    &   0.9      &   75.7   \\
\hline
EfficientFormer~\cite{efficientformer} & 3.1 & 0.9 & 74.2 \\
\rowcolor[gray]{0.92}
EfficientFormerV2 (Ours) &3.1 & 0.9 & 75.0 \\ 
% EfficientFormer~\cite{efficientformer} & 6.9 & 1.2 & 79.1 \\ 
% \rowcolor[gray]{0.92}
% EfficientFormerV2 (Ours) &7.0 & 1.2 & 79.4 \\ 
\bottomrule
\end{tabular}}\label{tab:ablate_search}
\end{table}

==> iccv2023AuthorKit/tabs/supp_0_training.tex <==
\begin{table}[h]
\caption{Training hyper-parameters for ImageNet-1K classification task. The drop path rate is for the [S0, S1, S2, L] model series. }
\label{tab:hyperparam}
\centering
% \small
\begin{tabular}{cc}
\toprule
Hyperparameters & Config                \\
\hline
optimizer       & AdamW                 \\
learning rate   & $0.001\times$(BS/$1024$)     \\
LR schedule     & cosine                \\
warmup epochs   & $5$                     \\
training epochs & $300$                   \\
weight decay    & $0.025$                 \\
augmentation    & RandAug($9$, $0.5$)       \\
color jitter    & $0.4$                   \\
gradient clip   & $0.01$                  \\
random erase    & $0.25$                  \\
label smooth     & $0.1$                   \\
mixup           & $0.8$                   \\
cutmix          & $1.0$                   \\
drop path       & {[}$0, 0, 0.02, 0.1${]} \\
\bottomrule
\end{tabular}
\end{table}

==> iccv2023AuthorKit/tabs/supp_1_longer_epoch.tex <==
\begin{table}[]

\caption{Analysis of explicit position encoding (Attention Bias). We use EfficientFormerV2-S1 for the experiments.}
\label{tab:long_epoch}
% \small
\centering
% \resizebox{0.5\textwidth}{!}{
\begin{tabular}{cccc}
\toprule
 Params (M) & Epoch & Attention Bias & Top-1 (\%) \\
\hline
6.10       & 300   & Y    & 79.0       \\
6.08       & 300   & N    & 78.8       \\ \hline
6.10       & 450   & Y    & 79.7       \\
6.08       & 450   & N    & 79.5      \\
\bottomrule
\end{tabular}
% }
\end{table}


% \begin{table}[]

% \caption{Experiments on more training epochs and explicit position encoding (Attention Bias, A.B.). }
% \label{tab:long_epoch}
% % \small
% \centering
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{ccccc}
% \toprule
% Model                & Params (M) & Epoch & A.B. & Top-1 (\%) \\
% \hline
% EfficientFormerV2-S1 & 6.10       & 300   & Y    & 79.0       \\
% EfficientFormerV2-S1 & 6.08       & 300   & N    & 78.8       \\
% EfficientFormerV2-S1 & 6.10       & 450   & Y    & 79.7       \\
% EfficientFormerV2-S1 & 6.08       & 450   & N    & 79.5      \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

==> iccv2023AuthorKit/tabs/supp_3_searchalpha.tex <==
\begin{table}[h]
\centering
% \small
\caption{Analysis of the $\alpha_{latency}$ and $\alpha_{size}$ in search algorithm.}\label{tab:search_alpha}
% \label{tab_alpha}
\resizebox{1\linewidth}{!}{
% \setlength{\tabcolsep}{1mm}
\begin{tabular}{ccccc}
\toprule
$\alpha_{latency}$ & $\alpha_{size}$ & Params (M) & Latency & Top-1 (\%) \\
\hline
1.0       & 1.0    &    3.5    &   1.1 ms     &    77.0   \\
0.5       & 1.0    &    3.5    &  1.3 ms      &  77.3     \\
\hline
\rowcolor[gray]{0.92}
1.0       & 0.5    & 3.5    & 0.9 ms    & 75.7  \\
\bottomrule
\end{tabular}
}
\end{table}
% \end{wraptable}

==> iccv2023AuthorKit/tabs/supp_expansion_analysis.tex <==
\begin{table}[h]
\caption{Ablation analysis on expansion ratios. Varying expansion ratios lead to different results even with the same number of parameters. Latency is obtained on iPhone 12.}
\label{tab:ablate_expansion}
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{cccc}
\toprule
Expansion ratio & Params (M) & Latency (ms) & Top-1 (\%) \\
\hline
4         & 13.4       & 1.6          & 81.8       \\
2         & 13.4       & 1.6          & 81.6       \\
1         & 13.4       & 1.6          & 81.1      \\
\bottomrule
\end{tabular}}
\end{table}


==> iccv2023AuthorKit/tabs/supp_network_architecture.tex <==
\begin{table*}[ht]
% \centering
\caption{Architecture details of EfficientFormerV2.}
\label{tab:achitecture}
\begin{tabular}{c|c|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{Stage} & \multirow{2}{*}{Resolution} & \multirow{2}{*}{Type} & \multirow{2}{*}{Config} & \multicolumn{4}{c}{EfficientFormerV2}                                   \\ \cline{5-8}
                       &                             &                       &                         & S0                & S1                & S2            & L               \\
                       \hline
\multirow{4}{*}{stem}  & \multirow{2}{*}{$\frac{H}{2}\times \frac{W}{2}$}         & \multirow{2}{*}{\texttt{Conv}} & Kernel, Stride           & $3\times 3$, $2$            & $3\times 3$, $2$            & $3\times 3$, $2$        & $3\times 3$, $2$          \\ \cline{4-8}
                       &                             &                       & N, C                    & $1$, $16$             & $1$, $16$             & $1$, $16$         & $1$, $20$           \\ \cline{2-8}
                       & \multirow{2}{*}{$\frac{H}{4}\times \frac{W}{4}$}         & \multirow{2}{*}{\texttt{Conv}} & Kernel, Stride           & $3\times 3$, $2$            & $3\times 3$, $2$            & $3\times 3$, $2$        & $3\times 3$, $2$          \\ \cline{4-8}
                       &                             &                       & N, C                    & $1$, $32$             & $1$, $32$             & $1$, $32$         & $1$, $40$           \\
                       \hline
\multirow{2}{*}{1}     & \multirow{2}{*}{$\frac{H}{4}\times \frac{W}{4}$}         & \multirow{2}{*}{\texttt{FFN}}  & N, C                    & $2$, $32$             & $3$, $32$             & $4$, $32$         & $5$, $40$           \\ \cline{4-8}
                       &                             &                       & E                       & {[}$4,4${]}         & {[}$4,4,4${]}       & {[}$4,4,4,4${]} & {[}$4,4,4,4,4${]} \\
                       \hline
\multirow{2}{*}{2}     & \multirow{2}{*}{$\frac{H}{8}\times \frac{W}{8}$}         & \multirow{2}{*}{\texttt{FFN}}  & N, C                    & $2, 48$             & $3, 48$             & $4, 64$         & $5, 80$           \\ \cline{4-8}
                       &                             &                       & E                       & {[}$4,4${]}         & {[}$4,4,4${]}       & {[}$4,4,4,4${]} & {[}$4,4,4,4,4${]} \\
                       \hline
\multirow{3}{*}{3}     & \multirow{3}{*}{$\frac{H}{16}\times \frac{W}{16}$}        & \multirow{2}{*}{\texttt{FFN}}  & N, C                    & $6, 96$             & $9, 120$            & $12, 144$       & $15, 192$         \\  \cline{4-8}
                       &                             &                       & E                       & {[}$4,3,3,3,4,4${]} & {[}$4(\times5),3(\times4)${]}     & {[}$4(\times6),3(\times6)${]} & {[}$4(\times8),3(\times7)${]}   \\
                      \cline{3-8}
                       &                             & \texttt{MHSA}                  & N                       & $2$                 & $2$                 & $4$             & $6$               \\
                       \hline
\multirow{3}{*}{4}     & \multirow{3}{*}{$\frac{H}{32}\times \frac{W}{32}$}        & \multirow{2}{*}{\texttt{FFN}}  & N, C                    & $4, 176$            & $6, 224$            & $8, 288$        & $10, 384$         \\ \cline{4-8}
                       &                             &                       & E                       & {[}$4,3,3,4${]}     & {[}$4,4,3,3,4,4${]} & {[}$4(\times4),3(\times4)${]} & {[}$4(\times6), 3(\times4)${]}  \\
                       \cline{3-8}
                       &                             & \texttt{MHSA}                  & N                       & $2$                 & $2$                 & $4$             & $6$  \\
                       \bottomrule
\end{tabular}
\end{table*}

==> iccv2023AuthorKit/tabs/supp_search_analysis.tex <==
\begin{table}[h]
\caption{Ablation on search methods for depth, width, and expansion ratios. EfficientFormer~\cite{efficientformer} merely searches for depth and width. On top of EfficientFormer~\cite{efficientformer}, we perform network pruning to decide channel numbers for stage width and expansion ratios. Finally, we show the results of our search algorithm for jointly optimizing depth, width, and expansions. }
\label{tab:ablate_CE_search}
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{cccc}
\toprule
Method  & Params (M) & Latency (ms) & Top-1 (\%) \\
\hline
From EfficientFormer~\cite{efficientformer}   & 7.0        & 1.15         & 79.2       \\
From EfficientFormer~\cite{efficientformer} + Pruning & 7.0        & 1.15         & 79.2       \\
\rowcolor[gray]{0.92}
Ours    & 7.0        & 1.15         & 79.4       \\
\bottomrule
\end{tabular}}
\end{table}

==> iccv2023AuthorKit/tabs/supp_search_figure.tex <==

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/compare_search.pdf}  
    \caption{Comparisons between our search method (Ours) and the search pipeline from EfficientFormer~\cite{efficientformer} (denoted as V1-scale), starting from the same supernet trained on ImageNet-1K. }
    \label{fig:compare_search}
\end{figure}

==> sections/0_abstract.tex <==
\begin{abstract}
With the success of Vision Transformers (ViTs) in computer vision tasks, recent arts try to optimize the performance and complexity of ViTs to enable efficient deployment on mobile devices.
Multiple approaches are proposed to accelerate attention mechanism, improve inefficient designs, or incorporate mobile-friendly lightweight convolutions to form hybrid architectures.
However, ViT and its variants still have \emph{higher latency} or considerably \emph{more parameters} than lightweight CNNs, even true for the years-old MobileNet. 
In practice, latency and size are both crucial for efficient deployment on resource-constraint hardware. 
In this work, we investigate a central question, can transformer models run as fast as MobileNet and maintain a similar size? 
We revisit the design choices of ViTs and propose a novel supernet with low latency and high parameter efficiency. 
We further introduce a novel fine-grained joint search strategy for transformer models that can find efficient architectures by optimizing latency and number of parameters simultaneously. The proposed models, EfficientFormerV2, achieve $3.5\%$ higher top-1 accuracy than MobileNetV2 on ImageNet-1K with similar latency and parameters. This work demonstrate that properly designed and optimized vision transformers can achieve high performance even with MobileNet-level size and speed.
% \footnote{Code: ~\href{https://github.com/snap-research/EfficientFormer}{\color{urlcolor}{https://github.com/snap-research/EfficientFormer}}.}



\end{abstract}



==> tabs/3_segmentation.tex <==
\begin{table}[]
\centering
\small
\caption{\textbf{Semantic segmentation} on ADE20K. EfficientFormerV2 models are integrated as feature encoder in Semantic FPN.}
\begin{tabular}{c|c|c}
\toprule
Backbone             & Params (M) & mIoU \\
\hline
ResNet18             & 11.7 & 32.9 \\
PoolFormer-S12       & 12.0 & 37.2 \\
EfficientFormer-L1   & 12.3 & 38.9 \\
\rowcolor[gray]{0.92}
EfficientFormerV2-S2 & 12.6 & 39.5 \\
\bottomrule
\end{tabular}
\label{tab:ade20k}
\end{table}

==> tabs/4_ablation.tex <==
\begin{table}[]
\centering
\small
\caption{
% Ablation on the proposed fine-grained search with joint constraints on size and speed, from the same supernet in Tab.~\ref{tab:comparison}
\textbf{Ablation of search algorithms.} We achieve better results than random search and the coarse-grained, single objective search from EfficientFormer~\cite{efficientformer}. 
Latency is measured on iPhone 12.
}
% \begin{tabular}{ccc|ccc}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
% \multicolumn{3}{c|}{Search in \cite{efficientformer}} & \multicolumn{3}{c}{Ours} \\
% \hline
% Params   & Latency   & Top-1  & Params & Latency & Top-1 \\
% (M)      & (ms)      & (\%)   & (M)    & (ms)    & (\%)  \\
% \hline
% 6.9      & 1.15      & 79.1   & 7.0    & 1.15    & 79.4  \\
% 3.1      & 0.90      & 74.2   & 3.1    & 0.90    & 75.0  \\
Search Algorithm & Params (M)& Latency (ms) & Top-1 ($\%$) \\ \hline
Random 1    &    3.5    &   1.0   &   74.7 \\
Random 2    &    3.5    &   1.0   &    75.0  \\
\rowcolor[gray]{0.92}
EfficientFormerV2 (Ours) &    3.5    &   0.9      &   75.7   \\
\hline
EfficientFormer~\cite{efficientformer} & 3.1 & 0.9 & 74.2 \\
\rowcolor[gray]{0.92}
EfficientFormerV2 (Ours) &3.1 & 0.9 & 75.0 \\ 
% EfficientFormer~\cite{efficientformer} & 6.9 & 1.2 & 79.1 \\ 
% \rowcolor[gray]{0.92}
% EfficientFormerV2 (Ours) &7.0 & 1.2 & 79.4 \\ 
\bottomrule
\end{tabular}}
\label{tab:ablate_search}
\end{table}
